Populating the brown dwarf and stellar boundary: Five stars with transiting companions near the hydrogen-burning mass limit

We report the discovery of five transiting companions near the hydrogen-burning mass limit in close orbits around main sequence stars originally identified by the Transiting Exoplanet Survey Satellite (TESS) as TESS Objects of Interest (TOIs): TOI-148, TOI-587, TOI-681, TOI-746, and TOI-1213. Using TESS and ground-based photometry as well as radial velocities from the CORALIE, CHIRON, TRES, and FEROS spectrographs, we found the companions have orbital periods between 4.8 and 27.2 days, masses between 77 and 98 $\mathrm{M_{Jup}}$, and radii between 0.81 and 1.66 $\mathrm{R_{Jup}}$. These targets have masses near the uncertain lower limit of hydrogen core fusion ($\sim$73-96 $\mathrm{M_{Jup}}$), which separates brown dwarfs and low-mass stars. We constrained young ages for TOI-587 (0.2 $\pm$ 0.1 Gyr) and TOI-681 (0.17 $\pm$ 0.03 Gyr) and found them to have relatively larger radii compared to other transiting companions of a similar mass. Conversely we estimated older ages for TOI-148 and TOI-746 and found them to have relatively smaller companion radii. With an effective temperature of 9800 $\pm$ 200 K, TOI-587 is the hottest known main-sequence star to host a transiting brown dwarf or very low-mass star. We found evidence of spin-orbit synchronization for TOI-148 and TOI-746 as well as tidal circularization for TOI-148. These companions add to the population of brown dwarfs and very low-mass stars with well measured parameters ideal to test formation models of these rare objects, the origin of the brown dwarf desert, and the distinction between brown dwarfs and hydrogen-burning main sequence stars.

==> tables/SG1obs_sub2.tex <==
\begin{table*}
\centering
    \begin{tabular}{llllll}
    \hline\hline
    Telescope & Location & Date & Filter & Aperture radius & Coverage\\
           &           & [UTC]&        &   [arcsec]      & \\
    \hline

%n20200607.Sloani.LCO-SAAO.dat && ingress && ip && Schwarz
%n20200627.Sloani.LCO-SSO.dat && ingress && ip && Schwarz  TTF: "This observation used Will Waalkes time.”— do we need to acknowledge that?
%n20200702.Sloani.LCO-SSO.dat && egress && ip && Schwarz
%n20200712.R.El-Sauce.dat && full && Rc && Phil Evans
%n20200721.Sloani.LCO-SAAO.dat && full && ip && Schwarz+Collins

{\it  TOI 148.01 (TIC 393940766)}\\
\hline
LCO-SAAO 1m    & South Africa   & 2020-06-07   &  $i^\prime$   & 4.7 & ingress \\
LCO-SSO 1m     & Australia      & 2020-06-27   &  $i^\prime$   & 5.1 & ingress \\
LCO-SSO 1m     & Australia      & 2020-07-02   &  $i^\prime$   & 4.7 & egress  \\
El-Sauce 0.36m & Chile          & 2020-07-12   &  $R_c$        & 5.9 & full \\
LCO-SAAO 1m    & South Africa   & 2020-07-21   &  $i^\prime$   & 4.3 & full \\[2mm] 

\hline

%n20191026.I.Brierfield.dat && full && I && Don Radford
%n20191126.I.CHAT.dat && egress && i && Rafael Brahm and CHAT
%n20191127.B.ElSauce.dat && full && B && Phil Evans
%n20200401.Sloang.MtStuart.dat && full && g && wingham
%n20200619.R.ASTEP.dat && full && Rc && mekarnia
{\it  TOI 681.01 (TIC 410450228)}\\
\hline
Brierfield 0.36m & Australia      & 2019-10-26  & I            & 10.3  & full \\
CHAT 0.7m        & Chile          & 2019-11-26  & $i^\prime$   & 8.4   & egress \\
El Sauce 0.36m   & Chile          & 2019-11-27  & B            & 7.4   & full \\
Mt. Stuart 0.32m & New Zealand    & 2020-04-01  & $g^\prime$   & 4.4   & full \\
ASTEP 0.4m       & Antarctica     & 2020-06-19  & $R_c$        & 10.2  & full \\[2mm] 

\hline
%n20190218.Sloanz.LCO-SAAO-1m.dat && ingress && zs  && Kevin Collins and Karen Collins
%n20190301.Sloanu.LCO-SAAO-1m.dat && full && up && Kevin Collins and Karen Collins
%n20190425.Sloanz.LCO-SAAO-1m.dat && ingress && zs && Kevin Collins and Karen Collins
%n20201025.V.PEST.dat && full && V && TG Tan
{\it  TOI 746.01 (TIC 167418903)}\\
\hline
LCO-SAAO 1m & South Africa        &  2019-02-18  & $z^\prime$   & 6.2   & ingress \\
LCO-SAAO 1m & South Africa        &  2019-03-01  & $u^\prime$   & 5.9   & full \\
LCO-SAAO 1m & South Africa        &  2019-04-25  & $z^\prime$   & 5.9   & ingress \\
PEST 0.31m  & Australia           &  2020-10-25  & V            & 7.4   & full \\[2mm] 

\hline
%n20200223.Sloani.Mearth.dat && full && RG715 && Jonathan Irwin
{\it TOI 1213.01 (TIC 399144800)}\\
\hline
MEarth-S 0.4m & Chile               &  2020-02-23  &  RG715       & 5.0   & full\\
ASTEP 0.4m       & Antarctica     & 2020-08-04  & $R_c$        & 10.2  & full \\[2mm]


\hline
\end{tabular}
\caption{Summary of Ground-based Photometric Follow-up Observations. Observatory acronyms: ASTEP--Antarctic Search for Transiting ExoPlanets; CHAT--Chilean-Hungarian Automated Telescope; LCO--Las Cumbres Observatory;  PEST--Perth Exoplanet Survey Telescope}
\label{table:SG1-obs}
\end{table*}






==> tables/oldtables/TOI-1213_param_old.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 10:52:47.72 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:23:14.9 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.54 \\
$A_V$ & V-band extinction (mag) & SED Fit & $0.12^{+0.00}_{-0.03}$ \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 6.197$\pm$0.014 \\
$d$ & Distance (pc) & SED Fit & ? \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 4.0$\pm$1.2 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.90^{+0.05}_{-0.04}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.990,0.041]}}$ & $1.01^{+0.03}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.82^{+0.13}_{-0.11}$ \\
$\rho_*$ & Density (cgs) & - & $1.24^{+0.15}_{-0.11}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.39^{+0.04}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5430,215]}}$ & $5480^{+160}_{-160}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.05,0.10]}}$ & $-0.02^{+0.10}_{-0.10}$ \\
$Age$ & Age (Gyr) & - & $10.7^{+2.3}_{-3.7}$ \\
$EEP$ & Equal Evolutionary Point & - & $401^{+12}_{-26}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $91.6^{+3.5}_{-2.5}$ \\
$R_B$ & Radius (\rj) & [0,2.5] & $1.55^{+0.63}_{-0.50}$ \\
$P$ & Period (days) & - & $27.214050^{+0.000200}_{-0.000200}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458576.19010^{+0.00180}_{-0.00180}$ \\
$a$ & Semi-major axis (AU) & - & $0.1762^{+0.0033}_{-0.0022}$ \\
$i$ & Inclination (Degrees) & - & $88.81^{+0.11}_{-0.10}$ \\
$e$ & Eccentricity & - & $0.4995^{+0.0055}_{-0.0047}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-63.3^{+0.4}_{-0.4}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $630^{+21}_{-22}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7212.0^{+57.0}_{-62.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.02500^{+0.02300}_{-0.01300}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.08510^{+0.00190}_{-0.00190}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.17020^{+0.00390}_{-0.00380}$ \\
$b$ & Transit Impact parameter & - & $1.057^{+0.069}_{-0.061}$ \\
$\rho_P$ & Density (cgs) & - & $30.0^{+69.0}_{-20.0}$ \\
log g$_P$ & Surface gravity & - & $4.980^{+0.340}_{-0.300}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.03^{+0.00}_{-0.00}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llcc}
\\
Wavelength Parameters & & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.481^{+0.050}_{-0.051} & 0.269^{+0.056}_{-0.054} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.361^{+0.047}_{-0.046} & 0.182^{+0.050}_{-0.049} \\ 
\end{tabular}
\\
%\begin{tabular}{llcc}
% \\ 
%Transit Parameters & & TESS 2-min & Mearth \\ 
%$\sigma^{2}$ & Added Variance & $-4.4e-07^{+7.1e-08}_{-6.7e-08} & 5.9e-06^{+2.4e-07}_{-2.3e-07} \\ 
%$F_0$ & Baseline flux & $1.00013^{+3.2e-05}_{-3.2e-05} & 1.00065^{+6.6e-05}_{-6.7e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llccc}
 \\ 
RV Parameters & & CHIRON & CORALIE & FEROS \\ 
$\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $24523^{+52}_{-53} & 25951^{+45}_{-47} & 25972^{+49}_{-47} \\ 
$\sigma_J$ & RV Jitter (m/s) & $60^{+28}_{-38} & 64^{+25}_{-37} & 52^{+31}_{-30} \\ 
$\sigma_J^2$ & RV Jitter Variance & $3600^{+4100}_{-3100} & 4200^{+3900}_{-3400} & 2800^{+4300}_{-2200} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-1213} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors and priors in brackets represent hard limit priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-1213}
\end{table*}


==> tables/oldtables/TOI-1213_param_sub1.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 1213, TIC 399144800, TYC 8970-00020-1, UCAC4 114-034370, 2MASS J10524799-6723161
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 10:52:47.72 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:23:14.9 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.54 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 6.197$\pm$0.014 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 4.0$\pm$1.2 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.97^{+0.07}_{-0.06}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.951,0.059]}}$ & $1.02^{+0.04}_{-0.05}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.89^{+0.15}_{-0.13}$ \\
$\rho_*$ & Density (cgs) & - & $1.27^{+0.22}_{-0.13}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.40^{+0.05}_{-0.04}$ \\
$T_{\rm eff}$ & Effective Temperature (K) & $\mathcal{G\text{[5675,175]}}$ & $5550^{+150}_{-150}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.28,0.16]}}$ & $0.25^{+0.14}_{-0.15}$ \\
$Age$ & Age (Gyr) & - & $7.9^{+3.8}_{-4.3}$ \\
$EEP$ & Equal Evolutionary Point & - & $387^{+22}_{-42}$ \\
\\
Companion Parameters & & & \\
$M_b$ & Mass (\mj) & - & $96.1^{+4.6}_{-3.7}$ \\
$R_b$ & Radius (\rj) & [0,3] & $1.54^{+0.99}_{-0.59}$ \\
$P$ & Period (days) & - & $27.214070^{+0.000200}_{-0.000200}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458576.19000^{+0.00180}_{-0.00180}$ \\
$a$ & Semi-major axis (AU) & - & $0.1806^{+0.0043}_{-0.0035}$ \\
$i$ & Inclination (Degrees) & - & $88.82^{+0.14}_{-0.15}$ \\
$e$ & Eccentricity & - & $0.4994^{+0.0030}_{-0.0027}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-63.2^{+0.3}_{-0.3}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $636^{+22}_{-23}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7203.0^{+29.0}_{-25.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.02300^{+0.03700}_{-0.01400}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.08480^{+0.00200}_{-0.00190}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.16960^{+0.00390}_{-0.00390}$ \\
$b$ & Transit Impact parameter & - & $1.052^{+0.110}_{-0.072}$ \\
$\rho_P$ & Density (cgs) & - & $33.0^{+110.0}_{-26.0}$ \\
log g$_P$ & Surface gravity & - & $5.010^{+0.420}_{-0.440}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.03^{+0.00}_{-0.00}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llcc}
\\
Wavelength Parameters & & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.485^{+0.050}_{-0.050}$ & $0.273^{+0.055}_{-0.054}$ \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.366^{+0.047}_{-0.047}$ & $0.187^{+0.050}_{-0.050}$ \\ 
\end{tabular}
\\
%\begin{tabular}{llcc}
% \\ 
%Transit Parameters & & TESS 2-min & Mearth \\ 
%$\sigma^{2}$ & Added Variance & $-4.3e-07^{+7.0e-08}_{-6.8e-08} & 6.0e-06^{+2.4e-07}_{-2.3e-07} \\ 
%$F_0$ & Baseline flux & $1.00013^{+3.2e-05}_{-3.2e-05} & 1.00065^{+6.9e-05}_{-6.8e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llccc}
 \\ 
RV Parameters & & CHIRON & CORALIE & FEROS \\ 
$\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $24529^{+20}_{-21}$ &$ 25956^{+38}_{-42}$ & $^{+36}_{-36} $\\ 
$\sigma_J$ & RV Jitter (m/s) & $46^{+30}_{-23}$ & $55^{+31}_{-38}$ & $53^{+30}_{-27}$ \\ 
$\sigma_J^2$ & RV Jitter Variance & $2200^{+3600}_{-1600}$ & $3100^{+4300}_{-2800}$ & $2800^{+4200}_{-2100} $\\ 
\hline
\end{tabular}
\caption{\textbf{TOI-1213} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors and priors in brackets represent hard limit priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-1213}
\end{table*}

==> tables/oldtables/TOI-1213_param_sub2_bad.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 1213, TIC 399144800, TYC 8970-00020-1, UCAC4 114-034370, 2MASS J10524799-6723161 
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 10:52:47.72 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:23:14.9 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.54 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 6.197$\pm$0.014 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 4.0$\pm$1.2 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.99^{+0.07}_{-0.07}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.951,0.059]}}$ & $0.99^{+0.04}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.87^{+0.14}_{-0.13}$ \\
$\rho_*$ & Density (cgs) & - & $1.42^{+0.19}_{-0.13}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.44^{+0.04}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5675,175]}}$ & $5600^{+150}_{-160}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.28,0.16]}}$ & $0.23^{+0.14}_{-0.14}$ \\
$Age$ & Age (Gyr) & - & $5.4^{+4.4}_{-3.4}$ \\
$EEP$ & Equal Evolutionary Point & - & $359^{+36}_{-30}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $97.6^{+4.4}_{-4.6}$ \\
$R_B$ & Radius (\rj) & [0,3] & $1.65^{+0.84}_{-0.55}$ \\
$P$ & Period (days) & - & $27.215260^{+0.000140}_{-0.000150}$ \\
$T_C$ & Time of conjunction (\bjdtdb) & - & $2458576.18680^{+0.00160}_{-0.00160}$ \\
$a$ & Semi-major axis (AU) & - & $0.1820^{+0.0041}_{-0.0043}$ \\
$i$ & Inclination (Degrees) & - & $88.85^{+0.12}_{-0.13}$ \\
$e$ & Eccentricity & - & $0.4981^{+0.0023}_{-0.0024}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-63.2^{+0.2}_{-0.2}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $629^{+21}_{-22}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7196.0^{+25.0}_{-20.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.02900^{+0.03400}_{-0.01500}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.08340^{+0.00160}_{-0.00170}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.16680^{+0.00310}_{-0.00330}$ \\
$b$ & Transit Impact parameter & - & $1.065^{+0.093}_{-0.067}$ \\
$\rho_P$ & Density (cgs) & - & $26.0^{+64.0}_{-19.0}$ \\
log g$_P$ & Surface gravity & - & $1.435^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.03^{+0.00}_{-0.00}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccc}
\\
Wavelength Parameters & & R & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & 0.476^{+0.054}_{-0.055} &0.312^{+0.051}_{-0.052} &0.338^{+0.054}_{-0.057} \\ 
$u_{2}$ & quadratic limb-darkening coeff & 0.300^{+0.050}_{-0.051} &0.232^{+0.050}_{-0.051} &0.250^{+0.051}_{-0.050} \\ 
\end{tabular}
\\
%\begin{tabular}{llccc}
% \\ 
%Transit Parameters & & TESS 2-min & Mearth & ASTEP \\ 
%$\sigma^{2}$ & Added Variance & -4.3e-07^{+6.8e-08}_{-6.9e-08} & 5.4e-06^{+2.2e-07}_{-2.2e-07} & 1.1e-06^{+2.0e-07}_{-2.0e-07} \\ 
%$F_0$ & Baseline flux & 0.95000^{+2.4e-01}_{-2.3e-01} & 1.00126^{+6.7e-05}_{-6.4e-05} & 0.99968^{+8.6e-05}_{-8.8e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llccc}
 \\ 
RV Parameters & & CHIRON & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & 24534^{+15}_{-17} & 25959^{+33}_{-35} & 25972^{+31}_{-34}  \\ 
$\sigma_J$ & RV Jitter (m/s) & 32^{+29}_{-20} & 49^{+30}_{-38} & 51^{+31}_{-25}  \\ 
$\sigma_J^2$ & RV Jitter Variance & 1060^{+2700}_{-890} & 2400^{+3900}_{-2300} & 2700^{+4100}_{-2000}  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-1213} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors and priors in brackets represent hard limit priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-1213}
\end{table*}

==> tables/oldtables/TOI-1213_param_withdilute.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 10:52:47.72 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:23:14.9 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.54 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 6.197$\pm$0.014 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 4.0$\pm$1.2 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.98^{+0.07}_{-0.06}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.951,0.059]}}$ & $0.99^{+0.04}_{-0.05}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.85^{+0.14}_{-0.13}$ \\
$\rho_*$ & Density (cgs) & - & $1.41^{+0.19}_{-0.13}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.43^{+0.04}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5675,175]}}$ & $5580^{+150}_{-160}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.28,0.16]}}$ & $0.24^{+0.14}_{-0.15}$ \\
$Age$ & Age (Gyr) & - & $6.0^{+4.3}_{-3.7}$ \\
$EEP$ & Equal Evolutionary Point & - & $365^{+31}_{-32}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $96.7^{+4.7}_{-4.2}$ \\
$R_B$ & Radius (\rj) & [0,3] & $1.73^{+0.82}_{-0.59}$ \\
$P$ & Period (days) & - & $27.215260^{+0.000150}_{-0.000150}$ \\
$T_C$ & Time of conjunction (\bjdtdb) & - & $2458576.18670^{+0.00180}_{-0.00160}$ \\
$a$ & Semi-major axis (AU) & - & $0.1812^{+0.0043}_{-0.0040}$ \\
$i$ & Inclination (Degrees) & - & $88.83^{+0.12}_{-0.12}$ \\
$e$ & Eccentricity & - & $0.4982^{+0.0025}_{-0.0023}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-63.2^{+0.2}_{-0.2}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $628^{+22}_{-22}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7198.0^{+23.0}_{-21.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.03200^{+0.03500}_{-0.01700}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.08330^{+0.00160}_{-0.00160}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.16660^{+0.00320}_{-0.00330}$ \\
$b$ & Transit Impact parameter & - & $1.075^{+0.090}_{-0.070}$ \\
$\rho_P$ & Density (cgs) & - & $23.0^{+57.0}_{-16.0}$ \\
log g$_P$ & Surface gravity & - & $1.435^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.03^{+0.00}_{-0.00}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccc}
\\
Wavelength Parameters & & R & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & 0.478^{+0.057}_{-0.058} &0.317^{+0.054}_{-0.057} &0.337^{+0.054}_{-0.054} \\ 
$u_{2}$ & quadratic limb-darkening coeff & 0.298^{+0.050}_{-0.048} &0.228^{+0.049}_{-0.049} &0.253^{+0.049}_{-0.051} \\ 
\end{tabular}
\\
%\begin{tabular}{llccc}
% \\ 
%Transit Parameters & & TESS 2-min & Mearth & ASTEP \\ 
%$\sigma^{2}$ & Added Variance & -4.4e-07^{+6.5e-08}_{-6.7e-08} & 5.4e-06^{+2.1e-07}_{-2.2e-07} & 1.1e-06^{+2.2e-07}_{-2.0e-07} \\ 
%$F_0$ & Baseline flux & 0.93000^{+2.0e-01}_{-2.0e-01} & 1.00125^{+7.2e-05}_{-7.3e-05} & 0.99967^{+8.5e-05}_{-8.1e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llccc}
 \\ 
RV Parameters & & CHIRON & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & 24535^{+15}_{-17} & 24535^{+15}_{-17} & 25952^{+37}_{-37}  \\ 
$\sigma_J$ & RV Jitter (m/s) & 34^{+31}_{-23} & 34^{+31}_{-23} & 48^{+34}_{-36}  \\ 
$\sigma_J^2$ & RV Jitter Variance & 1200^{+3100}_{-1100} & 1200^{+3100}_{-1100} & 2400^{+4400}_{-2200}  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-1213} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-1213}
\end{table*}

==> tables/oldtables/TOI-148_param_earlmar.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 148, TIC 393940766, UCAC4 260-199322, 2MASS J22331696-3809349 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 22:33:16.99 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -38:09:35.38 \\
$V_{mag}$ & V-band magnitude & TICv8 & 12.40 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 2.441\pm0.017 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & $10.1\pm0.8$ \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.96^{+0.12}_{-0.09}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[1.192,0.068]}}$ & $1.20^{+0.06}_{-0.07}$ \\
$L_*$ & Luminosity (\lsol) & - & $1.67^{+0.25}_{-0.23}$ \\
$\rho_*$ & Density (cgs) & - & $0.79^{+0.16}_{-0.12}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.26^{+0.06}_{-0.06}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5975,150]}}$ & $5990^{+140}_{-130}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.28,0.28]}}$ & $-0.26^{+0.26}_{-0.25}$ \\
$Age$ & Age (Gyr) & - & $8.0^{+3.6}_{-3.7}$ \\
$EEP$ & Equal Evolutionary Point & - & $419^{+16}_{-36}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $76.6^{+5.8}_{-4.4}$ \\
$R_B$ & Radius (\rj) & - & $0.77^{+0.05}_{-0.05}$ \\
$P$ & Period (days) & - & $4.867111^{+0.000013}_{-0.000018}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458327.32890^{+0.00260}_{-0.00180}$ \\
$a$ & Semi-major axis (AU) & - & $0.0569^{+0.0021}_{-0.0017}$ \\
$i$ & Inclination (Degrees) & - & $86.79^{+0.63}_{-0.54}$ \\
$e$ & Eccentricity & - & $0.0052^{+0.0060}_{-0.0037}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-62.0^{+85.0}_{-70.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $1325^{+47}_{-48}$ \\
$K$ & RV semi-amplitude (m/s) & - & $8950.0^{+50.0}_{-51.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.00435^{+0.00013}_{-0.00013}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.01240^{+0.00170}_{-0.00160}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.13740^{+0.00190}_{-0.00190}$ \\
$b$ & Transit Impact parameter & - & $0.573^{+0.060}_{-0.084}$ \\
$\rho_P$ & Density (cgs) & - & $207.0^{+48.0}_{-36.0}$ \\
log g$_P$ & Surface gravity & - & $5.505^{+0.064}_{-0.059}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.70^{+0.10}_{-0.10}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccc}
\\
Wavelength Parameters & & R & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.325^{+0.055}_{-0.055} & 0.256^{+0.033}_{-0.031} & 0.262^{+0.040}_{-0.039} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.312^{+0.051}_{-0.051} & 0.292^{+0.026}_{-0.026} & 0.290^{+0.035}_{-0.036} \\ 
\end{tabular}
\\
%\begin{tabular}{llccccccc}
% \\ 
%Transit Parameters & & TESS-FFI & TESS-2min & LCO-SAAO & LCO-SSO & LCO-SSO & El-Sauce & LCO-SAAO \\ 
%$\sigma^{2}$ & Added Variance & -4.7e-08^{+4.1e-08}_{-3.9e-08} & 4.0e-06^{+1.7e-07}_{-1.7e-07} & 1.1e-06^{+3.5e-07}_{-3.2e-07} & 2.4e-07^{+2.9e-07}_{-2.4e-07} & 1.0e-06^{+3.9e-07}_{-3.3e-07} & -8.7e-07^{+7.0e-07}_{-6.1e-07} & 6.4e-07^{+1.8e-07}_{-1.6e-07} \\ 
%$F_0$ & Baseline flux & 1.00004^{+3.0e-05}_{-3.1e-05} & 1.00017^{+3.3e-05}_{-3.3e-05} & 1.00007^{+1.2e-04}_{-1.2e-04} & 0.99988^{+1.4e-04}_{-1.4e-04} & 0.99993^{+1.5e-04}_{-1.6e-04} & 0.99884^{+2.5e-04}_{-2.5e-04} & 0.99971^{+9.3e-05}_{-9.5e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llc}
 \\ 
RV Parameters & & CORALIE & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & -29138^{+52}_{-53} \\ 
$\sigma_J$ & RV Jitter (m/s) & 69^{+22}_{-50} \\ 
$\sigma_J^2$ & RV Jitter Variance & 4900^{+3600}_{-4500} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-148} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-148}
\end{table*}

==> tables/oldtables/TOI-148_param_old.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 22:33:16.99 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -38:09:35.38 \\
$V_{mag}$ & V-band magnitude & TICv8 & 12.40 \\
$A_V$ & V-band extinction (mag) & SED Fit & $0.015\pm0.015$ \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 2.441\pm0.017 \\
$d$ & Distance (pc) & SED Fit & ? \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & $10.1\pm0.8$ \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.96^{+0.12}_{-0.08}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[1.216,0.055]}}$ & $1.22^{+0.05}_{-0.06}$ \\
$L_*$ & Luminosity (\lsol) & - & $1.67^{+0.31}_{-0.27}$ \\
$\rho_*$ & Density (cgs) & - & $0.75^{+0.13}_{-0.10}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.25^{+0.06}_{-0.05}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5836,286]}}$ & $5940^{+220}_{-210}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.28,0.28]}}$ & $-0.23^{+0.26}_{-0.26}$ \\
$Age$ & Age (Gyr) & - & $8.4^{+3.5}_{-4.0}$ \\
$EEP$ & Equal Evolutionary Point & - & $422^{+14}_{-34}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $76.7^{+6.0}_{-4.2}$ \\
$R_B$ & Radius (\rj) & - & $0.79^{+0.04}_{-0.04}$ \\
$P$ & Period (days) & - & $4.867112^{+0.000013}_{-0.000018}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458327.32890^{+0.00260}_{-0.00180}$ \\
$a$ & Semi-major axis (AU) & - & $0.0569^{+0.0022}_{-0.0016}$ \\
$i$ & Inclination (Degrees) & - & $86.65^{+0.54}_{-0.47}$ \\
$e$ & Eccentricity & - & $0.0052^{+0.0060}_{-0.0037}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-60.0^{+86.0}_{-69.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $1324^{+54}_{-56}$ \\
$K$ & RV semi-amplitude (m/s) & - & $8950.0^{+51.0}_{-52.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.00437^{+0.00013}_{-0.00012}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.01270^{+0.00150}_{-0.00140}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.13780^{+0.00180}_{-0.00180}$ \\
$b$ & Transit Impact parameter & - & $0.589^{+0.051}_{-0.068}$ \\
$\rho_P$ & Density (cgs) & - & $197.0^{+38.0}_{-30.0}$ \\
log g$_P$ & Surface gravity & - & $5.491^{+0.056}_{-0.052}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.70^{+0.12}_{-0.11}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccc}
\\
Wavelength Parameters & & R & Sloani & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.332^{+0.064}_{-0.060} & 0.262^{+0.042}_{-0.037} & 0.271^{+0.047}_{-0.044} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.307^{+0.051}_{-0.052} & 0.288^{+0.027}_{-0.028} & 0.288^{+0.036}_{-0.037} \\ 
\end{tabular}
\\
%\begin{tabular}{llccccccc}
% \\ 
%Transit Parameters & & TESS-FFI & TESS-2min & LCO-SAAO & LCO-SSO & LCO-SSO & El-Sauce & LCO-SAAO \\ 
%$\sigma^{2}$ & Added Variance & $-4.7e-08^{+4.1e-08}_{-3.9e-08} & 4.0e-06^{+1.7e-07}_{-1.7e-07} & 1.1e-06^{+3.6e-07}_{-3.2e-07} & 2.5e-07^{+2.9e-07}_{-2.4e-07} & 1.0e-06^{+3.9e-07}_{-3.3e-07} & -8.9e-07^{+7.0e-07}_{-6.0e-07} & 6.4e-07^{+1.9e-07}_{-1.7e-07} \\ 
%$F_0$ & Baseline flux & $1.00004^{+3.0e-05}_{-3.1e-05} & 1.00017^{+3.3e-05}_{-3.3e-05} & 1.00007^{+1.2e-04}_{-1.2e-04} & 0.99988^{+1.4e-04}_{-1.4e-04} & 0.99993^{+1.6e-04}_{-1.6e-04} & 0.99884^{+2.5e-04}_{-2.5e-04} & 0.99972^{+9.4e-05}_{-9.4e-05} \\ 
%\end{tabular}
%\\
\begin{tabular}{llc}
 \\ 
RV Parameters & & CORALIE & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $-29139^{+52}_{-54} \\ 
$\sigma_J$ & RV Jitter (m/s) & $70^{+22}_{-49} \\ 
$\sigma_J^2$ & RV Jitter Variance & $4900^{+3500}_{-4500} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-148} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-148}
\end{table*}


==> tables/oldtables/TOI-587_param_old.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 08:41:35.02 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -22:11:39.47 \\
$V_{mag}$ & V-band magnitude & TICv8 & 	7.8 \\
$A_V$ & V-band extinction (mag) & SED Fit & $0.02\pm0.02$ \\
$\varpi$ & Parallax (mas) & SED Fit & ? \\
$d$ & Distance (pc) & Gaia DR2 & 4.755$\pm$0.028 \\
\vsini & Surface Rotational Velocity (\kms) & TRES & 34.0$\pm$2.0 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $2.48^{+0.14}_{-0.13}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[2.024,0.088]}}$ & $2.00^{+0.09}_{-0.08}$ \\
$L_*$ & Luminosity (\lsol) & - & $42.20^{+6.50}_{-5.70}$ \\
$\rho_*$ & Density (cgs) & - & $0.44^{+0.06}_{-0.05}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.23^{+0.04}_{-0.04}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[10400,300]}}$ & $10390^{+300}_{-290}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.07,0.12]}}$ & $0.07^{+0.11}_{-0.12}$ \\
$Age$ & Age (Gyr) & - & $0.169^{+0.089}_{-0.075}$ \\
$EEP$ & Equal Evolutionary Point & - & $320^{+13}_{-19}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $84.2^{+6.1}_{-5.8}$ \\
$R_B$ & Radius (\rj) & - & $1.32^{+0.06}_{-0.06}$ \\
$P$ & Period (days) & - & $8.043460^{+0.000720}_{-0.000720}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458520.15888^{+0.00052}_{-0.00052}$ \\
$a$ & Semi-major axis (AU) & - & $0.1075^{+0.0020}_{-0.0019}$ \\
$i$ & Inclination (Degrees) & - & $88.11^{+0.89}_{-0.59}$ \\
$e$ & Eccentricity & - & $0.0400^{+0.0410}_{-0.0280}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $26.0^{+110.0}_{-95.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $2163^{+68}_{-67}$ \\
$K$ & RV semi-amplitude (m/s) & - & $4570.0^{+270.0}_{-270.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.00458^{+0.00008}_{-0.00008}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.01620^{+0.00230}_{-0.00190}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.22050^{+0.00200}_{-0.00180}$ \\
$b$ & Transit Impact parameter & - & $0.380^{+0.110}_{-0.180}$ \\
$\rho_P$ & Density (cgs) & - & $45.6^{+7.3}_{-6.4}$ \\
log g$_P$ & Surface gravity & - & $5.080^{+0.046}_{-0.049}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $4.95^{+0.65}_{-0.59}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llc}
\\
Wavelength Parameters & & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.135^{+0.057}_{-0.057} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.243^{+0.086}_{-0.085} \\ 
\end{tabular}
\\
%\begin{tabular}{llc}
% \\ 
%Transit Parameters & & TESS-FFI \\ 
%$\sigma^{2}$ & Added Variance & $1.0e-09^{+1.0e-09}_{-9.7e-10} \\ 
%$F_0$ & Baseline flux & $1.00000^{+5.2e-06}_{-5.1e-06} \\ 
%\end{tabular}
%\\
\begin{tabular}{llc}
 \\ 
RV Parameters & & TRES & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $-3290^{+250}_{-250} \\ 
$\sigma_J$ & RV Jitter (m/s) & $0^{+0}_{-0} \\ 
$\sigma_J^2$ & RV Jitter Variance & $-233000^{+140000}_{-93000} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-587} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-587}
\end{table*}

==> tables/oldtables/TOI-587_param_sub2_bad.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 587, TIC 294090620, HD 74162, HIP 42654, TYC 6024-00943-1, 2MASS J08413504-2211395 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 08:41:35.02 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -22:11:39.47 \\
$V_{mag}$ & V-band magnitude & TICv8 & 	7.8 \\
$\varpi$ & Parallax (mas) & Gaia DR2 & 4.755$\pm$0.028 \\
\vsini & Surface Rotational Velocity (\kms) & TRES & 34.0$\pm$2.0 \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $1.78^{+0.07}_{-0.07}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[2.031,0.092]}}$ & $2.15^{+0.08}_{-0.08}$ \\
$L_*$ & Luminosity (\lsol) & - & $35.10^{+4.20}_{-3.80}$ \\
$\rho_*$ & Density (cgs) & - & $0.25^{+0.03}_{-0.02}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.02^{+0.03}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[9800,200]}}$ & $9570^{+190}_{-200}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.07,0.12]}}$ & $-0.55^{+0.07}_{-0.07}$ \\
$Age$ & Age (Gyr) & - & $1.1^{+0.1}_{-0.1}$ \\
$EEP$ & Equal Evolutionary Point & - & $427^{+4}_{-3}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $67.1^{+5.8}_{-5.6}$ \\
$R_B$ & Radius (\rj) & - & $1.42^{+0.06}_{-0.05}$ \\
$P$ & Period (days) & - & $8.044245^{+0.000005}_{-0.000005}$ \\
$T_C$ & Time of conjunction (\bjdtdb) & - & $2458520.15795^{+0.00041}_{-0.00043}$ \\
$a$ & Semi-major axis (AU) & - & $0.0964^{+0.0013}_{-0.0012}$ \\
$i$ & Inclination (Degrees) & - & $86.49^{+0.27}_{-0.28}$ \\
$e$ & Eccentricity & - & $0.1240^{+0.0350}_{-0.0360}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $85.0^{+26.0}_{-25.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $2181^{+54}_{-53}$ \\
$K$ & RV semi-amplitude (m/s) & - & $4550.0^{+360.0}_{-370.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.00456^{+0.00003}_{-0.00003}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.01895^{+0.00086}_{-0.00083}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.22163^{+0.00074}_{-0.00074}$ \\
$b$ & Transit Impact parameter & - & $0.523^{+0.028}_{-0.031}$ \\
$\rho_P$ & Density (cgs) & - & $29.3^{+4.2}_{-3.7}$ \\
log g$_P$ & Surface gravity & - & $0.905^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $5.05^{+0.50}_{-0.46}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llc}
\\
Wavelength Parameters & & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & 0.199^{+0.052}_{-0.051}  \\ 
$u_{2}$ & quadratic limb-darkening coeff & 0.162^{+0.075}_{-0.072}  \\ 
\end{tabular}
\\
%\begin{tabular}{llc}
% \\ 
%Transit Parameters & & TESS-FFI \\ 
%$\sigma^{2}$ & Added Variance & 4.3e-08^{+1.2e-09}_{-1.2e-09} \\ 
%$F_0$ & Baseline flux & 1.00002^{+2.2e-06}_{-2.3e-06} \\ 
%\end{tabular}
%\\
\begin{tabular}{llc}
 \\ 
RV Parameters & & TRES & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & -3200^{+310}_{-310}  \\ 
$\sigma_J$ & RV Jitter (m/s) & 13^{+70}_{-14}  \\ 
$\sigma_J^2$ & RV Jitter Variance & 200^{+6800}_{-6900}  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-587} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-587}
\end{table*}

==> tables/oldtables/TOI-681_param_2feb.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 681, TIC 410450228, TYC 8911-00495-1, UCAC4 148-012283, 2MASS J07513479-6024448 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 07:51:34.79 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -60:24:44.6 \\
$V_{mag}$ & V-band magnitude & TICv8 & 10.885 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 2.442$\pm$0.013 \\
\vsini & Surface Rotational Velocity (\kms) & GALAH & $30.80\pm0.78$ \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $1.54^{+0.06}_{-0.05}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[1.586,0.067]}}$ & $1.48^{+0.04}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $6.05^{+0.66}_{-0.59}$ \\
$\rho_*$ & Density (cgs) & - & $0.67^{+0.05}_{-0.05}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.29^{+0.02}_{-0.02}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[7390,150]}}$ & $7430^{+140}_{-140}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.12,0.05]}}$ & $-0.08^{+0.05}_{-0.05}$ \\
$Age$ & Age (Gyr) & $\mathcal{G\text{[0.09,0.02]}}$ & $0.102^{+0.019}_{-0.020}$ \\
$EEP$ & Equal Evolutionary Point & - & $265^{+6}_{-7}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $88.9^{+2.5}_{-2.3}$ \\
$R_B$ & Radius (\rj) & [0,5] $ & $1.61^{+0.36}_{-0.19}$ \\
$P$ & Period (days) & - & $15.778363^{+0.000052}_{-0.000052}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458546.47724^{+0.00088}_{-0.00087}$ \\
$a$ & Semi-major axis (AU) & - & $0.1449^{+0.0018}_{-0.0016}$ \\
$i$ & Inclination (Degrees) & - & $87.59^{+0.10}_{-0.12}$ \\
$e$ & Eccentricity & - & $0.0980^{+0.0230}_{-0.0210}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-87.1^{+7.1}_{-5.4}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $1146^{+26}_{-25}$ \\
$K$ & RV semi-amplitude (m/s) & - & $5220.0^{+74.0}_{-70.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01240^{+0.00550}_{-0.00240}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.07250^{+0.00100}_{-0.00100}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.14490^{+0.00210}_{-0.00200}$ \\
$b$ & Transit Impact parameter & - & $0.966^{+0.034}_{-0.021}$ \\
$\rho_P$ & Density (cgs) & - & $26.0^{+12.0}_{-12.0}$ \\
log g$_P$ & Surface gravity & - & $4.930^{+0.110}_{-0.170}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.39^{+0.04}_{-0.03}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccccc}
\\
Wavelength Parameters & & B & I & R & Sloang & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.368^{+0.048}_{-0.049} & 0.177^{+0.034}_{-0.034} & 0.130^{+0.046}_{-0.046} & 0.372^{+0.045}_{-0.045} & 0.157^{+0.043}_{-0.044} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.340^{+0.049}_{-0.049} & 0.348^{+0.035}_{-0.035} & 0.276^{+0.047}_{-0.047} & 0.367^{+0.047}_{-0.047} & 0.326^{+0.045}_{-0.045} \\ 
\end{tabular}
\\
%\begin{tabular}{llcccccc}
% \\ 
%Transit Parameters & & TESS & Brierfield & CHAT & ElSauce & MtStuar & ASTEP \\ 
%$\sigma^{2}$ & Added Variance & $-1.1e-06^{+5.2e-08}_{-5.1e-08} & 2.6e-06^{+1.3e-06}_{-1.1e-06} & 1.4e-06^{+2.3e-07}_{-1.9e-07} & 7.4e-06^{+1.2e-06}_{-1.1e-06} & -7.0e-07^{+2.5e-07}_{-2.1e-07} & 2.8e-06^{+4.8e-07}_{-4.3e-07} \\ 
%$F_0$ & Baseline flux & $1.00008^{+2.7e-05}_{-2.7e-05} & 0.99884^{+3.0e-04}_{-3.0e-04} & 0.99958^{+1.3e-04}_{-1.3e-04} & 1.00229^{+2.5e-04}_{-2.5e-04} & 1.00233^{+2.6e-04}_{-2.6e-04} & 0.99886^{+1.7e-04}_{-1.8e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters & & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $22137^{+100}_{-93} & 23740^{+140}_{-140} \\ 
$\sigma_J$ & RV Jitter (m/s) & $95^{+3}_{-7} & 0^{+0}_{-0} \\ 
$\sigma_J^2$ & RV Jitter Variance & $9040^{+720}_{-1400} & -23000^{+21000}_{-16000} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-681} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors and priors in brackets represent hard limit priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-681}
\end{table*}

==> tables/oldtables/TOI-681_param_old.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 07:51:34.79 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -60:24:44.6 \\
$V_{mag}$ & V-band magnitude & TICv8 & 10.885 \\
$A_V$ & V-band extinction (mag) & SED Fit & $0.15\pm0.03$ \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 2.442$\pm$0.013 \\
$d$ & Distance (pc) & SED Fit & ? \\
\vsini & Surface Rotational Velocity (\kms) & GALAH & $30.80\pm0.78$ \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $1.56^{+0.05}_{-0.04}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[1.562,0.025]}}$ & $1.53^{+0.02}_{-0.02}$ \\
$L_*$ & Luminosity (\lsol) & - & $6.04^{+0.24}_{-0.23}$ \\
$\rho_*$ & Density (cgs) & - & $0.61^{+0.03}_{-0.03}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.26^{+0.01}_{-0.01}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[7297,45]}}$ & $7305^{+45}_{-45}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.122,0.051]}}$ & $-0.05^{+0.05}_{-0.05}$ \\
$Age$ & Age (Gyr) & $\mathcal{G\text{[0.09,0.02]}}$ & $0.106^{+0.019}_{-0.019}$ \\
$EEP$ & Equal Evolutionary Point & - & $266^{+6}_{-7}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $89.5^{+2.2}_{-2.0}$ \\
$R_B$ & Radius (\rj) & [0,5] $ & $1.92^{+0.61}_{-0.28}$ \\
$P$ & Period (days) & - & $15.778361^{+0.000053}_{-0.000053}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458546.47722^{+0.00089}_{-0.00090}$ \\
$a$ & Semi-major axis (AU) & - & $0.1454^{+0.0015}_{-0.0014}$ \\
$i$ & Inclination (Degrees) & - & $87.44^{+0.09}_{-0.12}$ \\
$e$ & Eccentricity & - & $0.0980^{+0.0240}_{-0.0210}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-87.1^{+7.2}_{-5.4}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $1144^{+11}_{-11}$ \\
$K$ & RV semi-amplitude (m/s) & - & $5219.0^{+76.0}_{-70.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01660^{+0.01200}_{-0.00430}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.07299^{+0.00099}_{-0.00099}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.14600^{+0.00200}_{-0.00200}$ \\
$b$ & Transit Impact parameter & - & $0.993^{+0.052}_{-0.028}$ \\
$\rho_P$ & Density (cgs) & - & $15.6^{+9.4}_{-8.7}$ \\
log g$_P$ & Surface gravity & - & $4.780^{+0.140}_{-0.240}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.39^{+0.01}_{-0.01}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccccc}
\\
Wavelength Parameters & & B & I & R & Sloang & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.378^{+0.046}_{-0.046} & 0.179^{+0.033}_{-0.033} & 0.131^{+0.045}_{-0.045} & 0.376^{+0.043}_{-0.044} & 0.161^{+0.043}_{-0.043} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.332^{+0.048}_{-0.048} & 0.353^{+0.034}_{-0.034} & 0.276^{+0.047}_{-0.047} & 0.360^{+0.046}_{-0.046} & 0.328^{+0.045}_{-0.044} \\ 
\end{tabular}
\\
%\begin{tabular}{llcccccc}
% \\ 
%Transit Parameters & & TESS & Brierfield & CHAT & ElSauce & MtStuar & ASTEP \\ 
%$\sigma^{2}$ & Added Variance & $-1.1e-06^{+5.3e-08}_{-5.0e-08} & 2.6e-06^{+1.3e-06}_{-1.1e-06} & 1.4e-06^{+2.2e-07}_{-1.9e-07} & 7.4e-06^{+1.2e-06}_{-1.1e-06} & -7.0e-07^{+2.4e-07}_{-2.1e-07} & 2.8e-06^{+4.8e-07}_{-4.3e-07} \\ 
%$F_0$ & Baseline flux & $1.00008^{+2.7e-05}_{-2.7e-05} & 0.99883^{+3.0e-04}_{-3.0e-04} & 0.99957^{+1.3e-04}_{-1.3e-04} & 1.00228^{+2.5e-04}_{-2.5e-04} & 1.00233^{+2.6e-04}_{-2.6e-04} & 0.99886^{+1.7e-04}_{-1.7e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters & & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $22136^{+100}_{-95} & 23740^{+140}_{-140} \\ 
$\sigma_J$ & RV Jitter (m/s) & $95^{+3}_{-7} & 0^{+0}_{-0} \\ 
$\sigma_J^2$ & RV Jitter Variance & $9030^{+720}_{-1400} & -23000^{+21000}_{-16000} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-681} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors and priors in brackets represent hard limit priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-681}
\end{table*}

==> tables/oldtables/TOI-681_param_withdilute.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 681, TIC 410450228, TYC 8911-00495-1, UCAC4 148-012283, 2MASS J07513479-6024448 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 07:51:34.79 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -60:24:44.6 \\
$V_{mag}$ & V-band magnitude & TICv8 & 10.885 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 2.442$\pm$0.013 \\
\vsini & Surface Rotational Velocity (\kms) & GALAH & $30.80\pm0.78$ \\
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $1.54^{+0.06}_{-0.05}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[1.586,0.067]}}$ & $1.47^{+0.04}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $6.02^{+0.60}_{-0.63}$ \\
$\rho_*$ & Density (cgs) & - & $0.68^{+0.05}_{-0.05}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.29^{+0.02}_{-0.02}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[7390,150]}}$ & $7450^{+140}_{-150}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[-0.12,0.05]}}$ & $-0.09^{+0.05}_{-0.04}$ \\
$Age$ & Age (Gyr) & $\mathcal{G\text{[0.09,0.02]}}$ & $0.1^{+0.0}_{-0.0}$ \\
$EEP$ & Equal Evolutionary Point & - & $265^{+6}_{-6}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $88.7^{+2.4}_{-2.2}$ \\
$R_B$ & Radius (\rj) & - & $1.47^{+0.19}_{-0.13}$ \\
$P$ & Period (days) & - & $15.778483^{+0.000026}_{-0.000027}$ \\
$T_C$ & Time of conjunction (\bjdtdb) & - & $2458546.47668^{+0.00066}_{-0.00069}$ \\
$a$ & Semi-major axis (AU) & - & $0.1448^{+0.0018}_{-0.0017}$ \\
$i$ & Inclination (Degrees) & - & $87.62^{+0.09}_{-0.10}$ \\
$e$ & Eccentricity & - & $0.0890^{+0.0190}_{-0.0180}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $-86.5^{+7.7}_{-5.9}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $1145^{+24}_{-27}$ \\
$K$ & RV semi-amplitude (m/s) & - & $5210.0^{+62.0}_{-64.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01040^{+0.00250}_{-0.00140}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.07175^{+0.00088}_{-0.00080}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.14350^{+0.00180}_{-0.00160}$ \\
$b$ & Transit Impact parameter & - & $0.953^{+0.019}_{-0.014}$ \\
$\rho_P$ & Density (cgs) & - & $34.0^{+11.0}_{-11.0}$ \\
log g$_P$ & Surface gravity & - & $1.198^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.39^{+0.03}_{-0.04}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccccc}
\\
Wavelength Parameters & & B & I & R & Sloang & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & 0.356^{+0.052}_{-0.046} &0.176^{+0.040}_{-0.038} &0.141^{+0.052}_{-0.047} &0.371^{+0.044}_{-0.048} &0.164^{+0.031}_{-0.031} \\ 
$u_{2}$ & quadratic limb-darkening coeff & 0.341^{+0.047}_{-0.054} &0.341^{+0.034}_{-0.035} &0.277^{+0.043}_{-0.042} &0.364^{+0.048}_{-0.047} &0.322^{+0.039}_{-0.038} \\ 
\end{tabular}
\\
%\begin{tabular}{llccccccc}
% \\ 
%Transit Parameters & & TESS FFI & TESS 2-min & Brierfield & CHAT & El Sauce & Mt Stuart & ASTEP \\ 
%$\sigma^{2}$ & Added Variance & 9.4e-08^{+2.7e-08}_{-2.3e-08} & -3.4e-07^{+3.2e-08}_{-3.2e-08} & 2.6e-06^{+1.3e-06}_{-1.0e-06} & 1.4e-06^{+2.0e-07}_{-1.9e-07} & 7.3e-06^{+1.3e-06}_{-1.1e-06} & -6.3e-07^{+2.9e-07}_{-2.2e-07} & 2.8e-06^{+4.5e-07}_{-3.8e-07} \\ 
%$F_0$ & Baseline flux & 1.00460^{+3.7e-03}_{-3.5e-03} & 1.00500^{+3.7e-03}_{-3.5e-03} & 0.99873^{+2.9e-04}_{-3.0e-04} & 0.99960^{+1.2e-04}_{-1.2e-04} & 1.00217^{+2.4e-04}_{-2.6e-04} & 1.00234^{+1.7e-04}_{-1.6e-04} & 0.99905^{+1.4e-04}_{-1.7e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters & & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & 22106^{+82}_{-85}  \\ 
$\sigma_J$ & RV Jitter (m/s) & 94^{+4}_{-7}  \\ 
$\sigma_J^2$ & RV Jitter Variance & 8850^{+820}_{-1400}  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-681} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-681}
\end{table*}

==> tables/oldtables/TOI-746_param_12feb.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 746, TIC 167418903, TYC 9177-00082-1, UCAC4 112-012172, 2MASS J06382899-6738563 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 06:38:28.99 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:38:56.22 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.807 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 4.167$\pm$0.014 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 6.1$\pm$1.2 \\
\\
\hline
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.93^{+0.09}_{-0.07}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.957,0.051]}}$ & $0.98^{+0.04}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.91^{+0.13}_{-0.11}$ \\
$\rho_*$ & Density (cgs) & - & $1.40^{+0.14}_{-0.14}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.43^{+0.03}_{-0.04}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5700,150]}}$ & $5690^{+140}_{-140}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.01,0.29]}}$ & $-0.03^{+0.23}_{-0.23}$ \\
$Age$ & Age (Gyr) & - & $7.2^{+4.1}_{-4.1}$ \\
$EEP$ & Equal Evolutionary Point & - & $376^{+27}_{-36}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $81.8^{+4.9}_{-4.2}$ \\
$R_B$ & Radius (\rj) & - & $0.99^{+0.12}_{-0.07}$ \\
$P$ & Period (days) & - & $10.980294^{+0.000028}_{-0.000028}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458335.77101^{+0.00074}_{-0.00074}$ \\
$a$ & Semi-major axis (AU) & - & $0.0970^{+0.0029}_{-0.0025}$ \\
$i$ & Inclination (Degrees) & - & $86.98^{+0.13}_{-0.18}$ \\
$e$ & Eccentricity & - & $0.1985^{+0.0029}_{-0.0031}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $116.5^{+1.0}_{-1.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $871^{+27}_{-26}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7565.0^{+21.0}_{-22.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01082^{+0.00190}_{-0.00092}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.04194^{+0.00075}_{-0.00091}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.08390^{+0.00140}_{-0.00140}$ \\
$b$ & Transit Impact parameter & - & $0.917^{+0.020}_{-0.013}$ \\
$\rho_P$ & Density (cgs) & - & $104.0^{+25.0}_{-30.0}$ \\
log g$_P$ & Surface gravity & - & $1.041^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.13^{+0.02}_{-0.01}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llcccc}
\\
Wavelength Parameters & & Sloanu & Sloanz & TESS & V \\ 
$u_{1}$ & linear limb-darkening coeff & 0.833^{+0.088}_{-0.095} &0.255^{+0.041}_{-0.042} &0.314^{+0.045}_{-0.045} &0.472^{+0.066}_{-0.065} \\ 
$u_{2}$ & quadratic limb-darkening coeff & 0.023^{+0.092}_{-0.088} &0.267^{+0.036}_{-0.036} &0.273^{+0.037}_{-0.036} &0.248^{+0.056}_{-0.057} \\ 
\end{tabular}
\\
%\begin{tabular}{llcccccc}
% \\ 
%Transit Parameters & & TESS-FFI & TESS 2-min & LCO-SAAO-1m & LCO-SAAO-1m & LCO-SAAO-1m & PEST \\ 
%$\sigma^{2}$ & Added Variance & 3.3e-07^{+4.5e-08}_{-4.3e-08} & 9.5e-07^{+1.3e-07}_{-1.3e-07} & 3.2e-06^{+9.1e-07}_{-7.8e-07} & 1.7e-06^{+1.1e-06}_{-8.8e-07} & 1.4e-07^{+2.1e-07}_{-1.7e-07} & 2.3e-06^{+1.5e-06}_{-1.2e-06} \\ 
%$F_0$ & Baseline flux & 1.00003^{+2.7e-05}_{-2.7e-05} & 0.99996^{+3.1e-05}_{-3.0e-05} & 1.00029^{+2.7e-04}_{-2.6e-04} & 0.99991^{+2.9e-04}_{-2.9e-04} & 1.00002^{+1.6e-04}_{-1.6e-04} & 1.00009^{+3.3e-04}_{-3.2e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters & & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & 33547^{+20}_{-21} & 33508^{+44}_{-43}  \\ 
$\sigma_J$ & RV Jitter (m/s) & 0^{+54}_{-0} & 61^{+27}_{-32}  \\ 
$\sigma_J^2$ & RV Jitter Variance & -400^{+3300}_{-1000} & 3800^{+4000}_{-2900}  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-746} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-746}
\end{table*}

==> tables/oldtables/TOI-746_param_old.tex <==
\begin{table*}
\centering
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 06:38:28.99 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:38:56.22 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.807 \\
%$A_V$ & V-band extinction (mag) & SED Fit & $0.07\pm0.03$ \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 4.167$\pm$0.014 \\
%$d$ & Distance (pc) & SED Fit & ? \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 6.1$\pm$1.2 \\
\\
\hline
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.87^{+0.05}_{-0.04}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.972,0.039]}}$ & $0.98^{+0.04}_{-0.04}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.81^{+0.11}_{-0.09}$ \\
$\rho_*$ & Density (cgs) & - & $1.31^{+0.14}_{-0.15}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.39^{+0.03}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5593,215]}}$ & $5550^{+91}_{-140}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.01,0.29]}}$ & $-0.20^{+0.09}_{-0.09}$ \\
$Age$ & Age (Gyr) & - & $10.0^{+3.1}_{-4.4}$ \\
$EEP$ & Equal Evolutionary Point & - & $397^{+15}_{-44}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $78.2^{+2.7}_{-2.1}$ \\
$R_B$ & Radius (\rj) & - & $1.04^{+0.14}_{-0.09}$ \\
$P$ & Period (days) & - & $10.980306^{+0.000044}_{-0.000041}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458335.77133^{+0.00094}_{-0.00098}$ \\
$a$ & Semi-major axis (AU) & - & $0.0948^{+0.0017}_{-0.0013}$ \\
$i$ & Inclination (Degrees) & - & $86.87^{+0.15}_{-0.20}$ \\
$e$ & Eccentricity & - & $0.1983^{+0.0035}_{-0.0024}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $116.6^{+0.9}_{-0.9}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $857^{+27}_{-26}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7569.0^{+20.0}_{-20.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01190^{+0.00220}_{-0.00140}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.04241^{+0.00069}_{-0.00077}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.08480^{+0.00140}_{-0.00150}$ \\
$b$ & Transit Impact parameter & - & $0.928^{+0.022}_{-0.016}$ \\
$\rho_P$ & Density (cgs) & - & $87.0^{+27.0}_{-27.0}$ \\
log g$_P$ & Surface gravity & - & $5.257^{+0.076}_{-0.110}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.12^{+0.01}_{-0.01}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llccc}
\\
Wavelength Parameters & & Sloanu & Sloanz & TESS \\ 
$u_{1}$ & linear limb-darkening coeff & $0.867^{+0.077}_{-0.057} & 0.260^{+0.049}_{-0.035} & 0.330^{+0.042}_{-0.042} \\ 
$u_{2}$ & quadratic limb-darkening coeff & $-0.003^{+0.065}_{-0.078} & 0.261^{+0.032}_{-0.035} & 0.262^{+0.042}_{-0.036} \\ 
\end{tabular}
\\
%\begin{tabular}{llccccc}
% \\ 
%Transit Parameters & & TESS-FFI & TESS 2-min & LCO-SAAO-1m & LCO-SAAO-1m & LCO-SAAO-1m \\ 
%$\sigma^{2}$ & Added Variance & $3.3e-07^{+4.0e-08}_{-3.8e-08} & 9.6e-07^{+1.2e-07}_{-1.3e-07} & 3.2e-06^{+9.4e-07}_{-8.2e-07} & 1.5e-06^{+9.6e-07}_{-1.0e-06} & 1.4e-07^{+2.2e-07}_{-1.7e-07} \\ 
%$F_0$ & Baseline flux & $1.00003^{+2.2e-05}_{-2.7e-05} & 0.99996^{+3.5e-05}_{-2.5e-05} & 1.00014^{+5.0e-04}_{-7.7e-04} & 0.99879^{+4.8e-04}_{-8.5e-04} & 1.00023^{+4.9e-04}_{-4.1e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters & & CORALIE & FEROS & $\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $33547^{+23}_{-24} & 33512^{+47}_{-40} \\ 
$\sigma_J$ & RV Jitter (m/s) & $0^{+51}_{-0} & 69^{+21}_{-32} \\ 
$\sigma_J^2$ & RV Jitter Variance & $-600^{+3200}_{-880} & 4800^{+3400}_{-3400} \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-746} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-746}
\end{table*}

==> tables/oldtables/TOI-746_param_old_mar2021.tex <==
\begin{table*}
\centering
Star Name \& Aliases: TOI 746, TIC 167418903, TYC 9177-00082-1, UCAC4 112-012172, 2MASS J06382899-6738563 \\
\begin{tabular}{llcc}
\hline\hline
Parameter & Unit & Source & Value \\
\hline
Stellar Parameters & & & \\
$\alpha$ & Right Ascension \text{(hh:mm:ss)} & TICv8 & 06:38:28.99 \\
$\delta$ & Declination \text{(deg:min:sec)} & TICv8 & -67:38:56.22 \\
$V_{mag}$ & V-band magnitude & TICv8 & 11.807 \\
$\varpi$ & Parallax (mas) & GAIA DR2 & 4.167$\pm$0.014 \\
\vsini & Surface Rotational Velocity (\kms) & CORALIE & 6.1$\pm$1.2 \\
\\
\hline
\\
\hline
Parameter & Unit & Exofast & Value \\
 & & Priors & \\
\hline
\\
$M_*$ & Mass (\msol) & - & $0.93^{+0.09}_{-0.07}$ \\ 
$R_*$ & Radius (\rsol) & $\mathcal{G\text{[0.957,0.051]}}$ & $0.98^{+0.04}_{-0.03}$ \\
$L_*$ & Luminosity (\lsol) & - & $0.91^{+0.13}_{-0.11}$ \\
$\rho_*$ & Density (cgs) & - & $1.41^{+0.12}_{-0.12}$ \\
$\log{g}$ & Surface gravity (cgs) & - & $4.43^{+0.03}_{-0.03}$ \\
$T_{\rm eff}$ &Effective Temperature (K) & $\mathcal{G\text{[5700,150]}}$ & $5690^{+140}_{-140}$ \\
$[{\rm Fe/H}]$ &Metallicity (dex) & $\mathcal{G\text{[0.01,0.29]}}$ & $-0.03^{+0.23}_{-0.23}$ \\
$Age$ & Age (Gyr) & - & $7.0^{+4.1}_{-4.0}$ \\
$EEP$ & Equal Evolutionary Point & - & $374^{+27}_{-35}$ \\
\\
Companion Parameters & & & \\
$M_B$ & Mass (\mj) & - & $81.9^{+4.9}_{-4.2}$ \\
$R_B$ & Radius (\rj) & - & $0.99^{+0.09}_{-0.06}$ \\
$P$ & Period (days) & - & $10.980303^{+0.000011}_{-0.000011}$ \\
$T_C$ & Time of conjunction - 2450000 (\bjdtdb) & - & $2458335.77070^{+0.00052}_{-0.00052}$ \\
$a$ & Semi-major axis (AU) & - & $0.0971^{+0.0029}_{-0.0025}$ \\
$i$ & Inclination (Degrees) & - & $86.99^{+0.11}_{-0.15}$ \\
$e$ & Eccentricity & - & $0.1985^{+0.0029}_{-0.0031}$ \\
$\omega_*$ & Argument of Periastron (Degrees) & - & $116.5^{+1.0}_{-1.0}$ \\
$T_{eq}$ & Equilibrium temperature (K) & - & $871^{+26}_{-25}$ \\
$K$ & RV semi-amplitude (m/s) & - & $7565.0^{+21.0}_{-22.0}$ \\
$\delta$ & Transit depth (fraction) & - & $0.01080^{+0.00150}_{-0.00076}$ \\
$\tau$ & Ingress/egress transit duration (days) & - & $0.04209^{+0.00063}_{-0.00070}$ \\
$T_{14}$ & Total transit duration (days) & - & $0.08420^{+0.00120}_{-0.00120}$ \\
$b$ & Transit Impact parameter & - & $0.915^{+0.016}_{-0.011}$ \\
$\rho_P$ & Density (cgs) & - & $105.0^{+20.0}_{-25.0}$ \\
log g$_P$ & Surface gravity & - & $1.041^{+0.000}_{-0.000}$ \\
$\fave$ & Incident Flux (\fluxcgs) & - & $0.13^{+0.02}_{-0.01}$ \\
\hline
\end{tabular}
\\
\begin{tabular}{llcccc}
\\
Wavelength Parameters & & Sloanu & Sloanz & TESS & V \\ 
$u_{1}$ & linear limb-darkening coeff & $0.835^{+0.088}_{-0.094}$ &$0.257^{+0.041}_{-0.041}$ &$0.308^{+0.044}_{-0.044}$ &$0.471^{+0.066}_{-0.066}$ \\ 
$u_{2}$ & quadratic limb-darkening coeff & $0.026^{+0.091}_{-0.088}$ &$0.268^{+0.036}_{-0.036}$ &$0.268^{+0.036}_{-0.036}$ &$0.248^{+0.056}_{-0.056}$ \\ 
\end{tabular}
\\
%\begin{tabular}{llcccccc}
% \\ 
%Transit Parameters & & TESS-FFI & TESS 2-min & LCO-SAAO-1m & LCO-SAAO-1m & LCO-SAAO-1m & PEST \\ 
%$\sigma^{2}$ & Added Variance & -4.7e-08^{+4.0e-08}_{-3.7e-08} & 3.9e-06^{+8.9e-08}_{-8.9e-08} & 3.2e-06^{+9.3e-07}_{-7.7e-07} & 1.7e-06^{+1.1e-06}_{-8.8e-07} & 1.3e-07^{+2.1e-07}_{-1.7e-07} & 2.2e-06^{+1.5e-06}_{-1.2e-06} \\ 
%$F_0$ & Baseline flux & 1.00002^{+2.7e-05}_{-2.7e-05} & 1.00004^{+2.0e-05}_{-2.0e-05} & 1.00035^{+2.6e-04}_{-2.6e-04} & 0.99994^{+2.9e-04}_{-2.9e-04} & 1.00007^{+1.6e-04}_{-1.6e-04} & 1.00013^{+3.2e-04}_{-3.2e-04} \\ 
%\end{tabular}
%\\
\begin{tabular}{llcc}
 \\ 
RV Parameters && CORALIE & FEROS \\
$\gamma_{\rm rel}$ & Relative RV Offset (m/s) & $33547^{+20}_{-21}$ & $33509^{+44}_{-44}$  \\ 
$\sigma_J$ & RV Jitter (m/s) & $0^{+53}_{-0}$ & $62^{+26}_{-31}$  \\ 
$\sigma_J^2$ & RV Jitter Variance & $-430^{+3200}_{-1000}$ & $3900^{+4000}_{-2900}$  \\ 
\hline
\end{tabular}
\caption{\textbf{TOI-746} stellar and companion parameters. Priors are for the EXOFASTv2 global model only, where $\mathcal{G\text{[a,b]}}$ are Gaussian priors. The topmost parameters were not modeled with EXOFASTv2 and the source of their value is displayed.}
\label{tab:TOI-746}
\end{table*}

==> tables/oldtables/sed_table.tex <==
\begin{sidewaystable} 
   \centering\small
    %\hspace*{-1cm}
%    \begin{adjustbox}{angle=90}
    \begin{tabular}{cccccccccccccc}
        \hline\hline
        Star & $\chi_\nu^2$ & $\teff$ & $\feh$ & $\logg$  & $A_V$  &  $F_{\rm bol}$ & $R_\star$  &  $M_\star^a$ &  $M_\star^b$  &  $P_{\rm rot}/\sin i$  &  $\tau_\star^c$  &  $R'_{\rm HK}$  & $\tau_\star^d$  \\
         &  &  [K] & dex & dex & mag & $10^{-10}$ [erg~s$^{-1}$~cm$^{-2}$] & R$_\odot$ & M$_\odot$  & M$_\odot$ & [d]  & [Gyr]  & dex  & [Gyr] \\
        \hline
        TOI-148 & 1.4 & 5975 $\pm$ 150 & -0.50 $\pm$ 0.25 & 4.25 $\pm$ 0.1 & 0.03 $\pm$ 0.03 & 3.405 $\pm$ 0.079 & 1.192 $\pm$ 0.068 & 0.94 $\pm$ 0.26 & 1.03 $\pm$ 0.06 & 5.97 $\pm$ 0.47 & 0.55 $\pm$ 0.07 & -- & -- \\     
        TOI-587 & 0.9 & 9800 $\pm$ 200 & -0.10 $\pm$ 0.15 & 4.15 $\pm$ 0.15 & 0.02 $\pm$ 0.02 & 252.9 $\pm$ 5.9 & 2.031 $\pm$ 0.092 & 2.12 $\pm$ 0.29 & 2.32 $\pm$ 0.14 & 3.02 $\pm$ 0.18 & -- & -- & -- \\  
        TOI-681 & 1.0 & 7390 $\pm$ 150 & -0.25 $\pm$ 0.25 & 4.20 $\pm$ 0.15 & 0.22 $\pm$ 0.02 & 12.41 $\pm$ 0.14 & 1.586 $\pm$ 0.067 & 1.45 $\pm$ 0.25 & 1.51 $\pm$ 0.09 & 2.61 $\pm$ 0.13 & -- & -- & -- \\  
        TOI-746 & 1.6 & 5700 $\pm$ 150 & -0.25 $\pm$ 0.25 & 4.40 $\pm$ 0.10 & 0.18 $\pm$ 0.02 & 5.126 $\pm$ 0.059 & 0.957 $\pm$ 0.051 & 0.84 $\pm$ 0.12 & 0.98 $\pm$ 0.06 & 7.9 $\pm$ 1.6 & 0.52 $\pm$ 0.06 & $-4.50 \pm 0.05$ & 0.60 $\pm$ 0.23 \\  
        TOI-1213 & 1.2 & 5675 $\pm$ 175 & 0.00 $\pm$ 0.25 & 4.45 $\pm$ 0.10 & 0.34 $\pm$ 0.03 & 10.47 $\pm$ 0.12 & 0.951 $\pm$ 0.059 & 0.93 $\pm$ 0.15 & 1.01 $\pm$ 0.06 & 12.0 $\pm$ 3.6 & 1.1 $\pm$ 0.2 & -- & -- \\  
        \hline
        %Santos CORALIE vsini estimates:
        %TOI-148 & 7.1 $\pm$ 0.8
        %TOI-746 & $<$ 2.5
        %TOI-1213 & $<$ 2.5
    \end{tabular}
%    \end{adjustbox}
    \caption{Table of stellar parameters derived from SED fitting and empirical relations. $^a$Stellar mass inferred from $R_\star$ and spectroscopic \logg. $^b$Stellar mass estimated via empirical relations of \citet{Torres2010}. $^c$System age estimated from inferred rotation period via empirical relations of \citet{Mamajek:2008}. $^d$System age estimated from inferred $R'_{\rm HK}$ via empirical relations of \citet{Mamajek:2008}.}
    \label{tab:sed}
\end{sidewaystable}


==> tables/oldtables/sed_table_copy.tex <==
\begin{sidewaystable} 
   %\centering\small
   \centering\tiny
    %\hspace*{-1cm}
%    \begin{adjustbox}{angle=90}
    \begin{tabular}{cccccccccccccc}
        \hline\hline
        Star & $\chi_\nu^2$ & $\teff$ & $\feh$ & $\logg$  & $A_V$  &  $F_{\rm bol}$ & $R_\star$  &  $M_\star^a$ &  $M_\star^b$  &  $P_{\rm rot}/\sin i$  &  $\tau_\star^c$  &  $R'_{\rm HK}$  & $\tau_\star^d$  \\
         &  &  [K] & dex & dex & mag & $10^{-10}$ [erg~s$^{-1}$~cm$^{-2}$] & R$_\odot$ & M$_\odot$  & M$_\odot$ & [d]  & [Gyr]  & dex  & [Gyr] \\
        \hline
        TOI-148 & 1.4 & 5975 $\pm$ 150 & -0.50 $\pm$ 0.25 & 4.25 $\pm$ 0.1 & 0.03 $\pm$ 0.03 & 3.405 $\pm$ 0.079 & 1.192 $\pm$ 0.068 & 0.94 $\pm$ 0.26 & 1.03 $\pm$ 0.06 & 5.97 $\pm$ 0.47 & 0.55 $\pm$ 0.07 & -- & -- \\     
        TOI-587 & 0.9 & 9800 $\pm$ 200 & -0.10 $\pm$ 0.15 & 4.15 $\pm$ 0.15 & 0.02 $\pm$ 0.02 & 252.9 $\pm$ 5.9 & 2.031 $\pm$ 0.092 & 2.12 $\pm$ 0.29 & 2.32 $\pm$ 0.14 & 3.02 $\pm$ 0.18 & -- & -- & -- \\  
        TOI-681 & 1.0 & 7390 $\pm$ 150 & -0.25 $\pm$ 0.25 & 4.20 $\pm$ 0.15 & 0.22 $\pm$ 0.02 & 12.41 $\pm$ 0.14 & 1.586 $\pm$ 0.067 & 1.45 $\pm$ 0.25 & 1.51 $\pm$ 0.09 & 2.61 $\pm$ 0.13 & -- & -- & -- \\  
        TOI-746 & 1.6 & 5700 $\pm$ 150 & -0.25 $\pm$ 0.25 & 4.40 $\pm$ 0.10 & 0.18 $\pm$ 0.02 & 5.126 $\pm$ 0.059 & 0.957 $\pm$ 0.051 & 0.84 $\pm$ 0.12 & 0.98 $\pm$ 0.06 & 7.9 $\pm$ 1.6 & 0.52 $\pm$ 0.06 & $-4.50 \pm 0.05$ & 0.60 $\pm$ 0.23 \\  
        TOI-1213 & 1.2 & 5675 $\pm$ 175 & 0.00 $\pm$ 0.25 & 4.45 $\pm$ 0.10 & 0.34 $\pm$ 0.03 & 10.47 $\pm$ 0.12 & 0.951 $\pm$ 0.059 & 0.93 $\pm$ 0.15 & 1.01 $\pm$ 0.06 & 12.0 $\pm$ 3.6 & 1.1 $\pm$ 0.2 & -- & -- \\  
        \hline
        %Santos CORALIE vsini estimates:
        %TOI-148 & 7.1 $\pm$ 0.8
        %TOI-746 & $<$ 2.5
        %TOI-1213 & $<$ 2.5
    \end{tabular}
%    \end{adjustbox}
    \caption{Table of stellar parameters derived from SED fitting and empirical relations. $^a$Stellar mass inferred from $R_\star$ and spectroscopic \logg. $^b$Stellar mass estimated via empirical relations of \citet{Torres2010}. $^c$System age estimated from inferred rotation period via empirical relations of \citet{Mamajek:2008}. $^d$System age estimated from inferred $R'_{\rm HK}$ via empirical relations of \citet{Mamajek:2008}.}
    \label{tab:sed}
\end{sidewaystable}


==> tables/oldtables/transiting_companions_table_sub1.tex <==
\begin{table*} 
\centering
List of Published 13-150 \mjup Transiting Companions as of April 2021
\tiny
%\hspace*{-0.25cm}
\begin{tabular}{lccrcccccc}
\hline\hline
Name & M$_{\rm2} [\mjup] & R$_{\rm2} [\rjup] & $P$ [days] & $ecc$ & M$_{\rm1} [\msol] & R$_{\rm1} [\rsol] & \teff [K] & \feh & Reference \\

\hline
HATS-70b & 12.9$_{-1.6}^{+1.8}$ & 1.38$_{-0.07}^{+0.08}$ & 1.89 & <0.18 & 1.78\,$\pm$\,0.12 & 1.88$_{-0.07}^{+0.06}$ & 7930$_{-820}^{+630}$ & 0.04$_{-0.11}^{+0.10}$ & (1) \\ 
GPX-1b & 19.7\,$\pm$\,1.6 & 1.47\,$\pm$\,0.10 & 1.74 & 0.000\,$\pm$\,0.000 & 1.68\,$\pm$\,0.10 & 1.56\,$\pm$\,0.10 & 7000\,$\pm$\,200 & 0.35\,$\pm$\,0.10 & (2) \\ 
Kepler-39b & 20.1$_{-1.2}^{+1.3}$ & 1.24$_{-0.10}^{+0.09}$ & 21.09 & 0.112\,$\pm$\,0.057 & 1.29$_{-0.07}^{+0.06}$ & 1.40\,$\pm$\,0.10 & 6350\,$\pm$\,100 & 0.10\,$\pm$\,0.14 & (3) \\ 
CoRoT-3b & 21.7\,$\pm$\,1.0 & 1.01\,$\pm$\,0.07 & 4.26 & 0 (fixed) & 1.37\,$\pm$\,0.09 & 1.56\,$\pm$\,0.09 & 6740\,$\pm$\,140 & -0.02\,$\pm$\,0.06 & (4) \\ 
KELT-1b & 27.4\,$\pm$\,0.9 & 1.12$_{-0.03}^{+0.04}$ & 1.22 & 0.010$_{-0.007}^{+0.010}$ & 1.33\,$\pm$\,0.06 & 1.47\,$\pm$\,0.04 & 6516\,$\pm$\,49 & 0.05\,$\pm$\,0.08 & (5) \\ 
NLTT 41135b & 33.7$_{-2.6}^{+2.8}$ & 1.13$_{-0.17}^{+0.27}$ & 2.89 & <0.02 & 0.19$_{-0.02}^{+0.03}$ & 0.21$_{-0.01}^{+0.02}$ & 3230\,$\pm$\,130 & -0.25\,$\pm$\,0.25 & (6) \\ 
WASP-128b & 37.2\,$\pm$\,0.8 & 0.94\,$\pm$\,0.02 & 2.21 & <0.007 & 1.16\,$\pm$\,0.04 & 1.15\,$\pm$\,0.02 & 5950\,$\pm$\,50 & 0.01\,$\pm$\,0.12 & (7) \\ 
CWW 89Ab & 39.2$_{-1.1}^{+0.9}$ & 0.94\,$\pm$\,0.02 & 5.29 & 0.189\,$\pm$\,0.002 & 1.10\,$\pm$\,0.04 & 1.03\,$\pm$\,0.02 & 5755\,$\pm$\,49 & 0.20\,$\pm$\,0.09 & (8) (9) \\ 
KOI-205b & 39.9\,$\pm$\,1.0 & 0.81\,$\pm$\,0.02 & 11.72 & <0.031 & 0.93\,$\pm$\,0.03 & 0.84\,$\pm$\,0.02 & 5237\,$\pm$\,60 & 0.14\,$\pm$\,0.12 & (10) \\ 
TOI-1406b & 46.0$_{-2.7}^{+2.6}$ & 0.86\,$\pm$\,0.03 & 10.57 & 0.026$_{-0.010}^{+0.013}$ & 1.18$_{-0.09}^{+0.08}$ & 1.35\,$\pm$\,0.03 & 6290\,$\pm$\,100 & -0.08\,$\pm$\,0.09 & (11) \\ 
EPIC 212036875b & 52.3\,$\pm$\,1.9 & 0.87\,$\pm$\,0.02 & 5.17 & 0.132\,$\pm$\,0.004 & 1.29$_{-0.06}^{+0.07}$ & 1.50\,$\pm$\,0.03 & 6238$_{-60}^{+59}$ & 0.01\,$\pm$\,0.10 & (9) (12) \\ 
TOI-503b & 53.7\,$\pm$\,1.2 & 1.34$_{-0.15}^{+0.26}$ & 3.68 & 0 (fixed) & 1.80\,$\pm$\,0.06 & 1.70$_{-0.04}^{+0.05}$ & 7650$_{-160}^{+140}$ & 0.30$_{-0.09}^{+0.08}$ & (13) \\ 
TOI-852b & 53.7$_{-1.3}^{+1.4}$ & 0.83\,$\pm$\,0.04 & 4.95 & 0.004$_{-0.003}^{+0.004}$ & 1.32$_{-0.04}^{+0.05}$ & 1.71\,$\pm$\,0.04 & 5768$_{-81}^{+84}$ & 0.33\,$\pm$\,0.09 & (14) \\ 
AD 3116b & 54.2\,$\pm$\,4.3 & 1.02\,$\pm$\,0.28 & 1.98 & 0.146\,$\pm$\,0.024 & 0.28\,$\pm$\,0.02 & 0.29\,$\pm$\,0.08 & 3184\,$\pm$\,29 & 0.16\,$\pm$\,0.10 & (15) \\ 
CoRoT-33b & 59.0$_{-1.7}^{+1.8}$ & 1.10\,$\pm$\,0.53 & 5.82 & 0.070\,$\pm$\,0.002 & 0.86\,$\pm$\,0.04 & 0.94$_{-0.08}^{+0.14}$ & 5225\,$\pm$\,80 & 0.44\,$\pm$\,0.10 & (16) \\ 
RIK 72b & 59.2$_{-6.7}^{+6.8}$ & 3.10\,$\pm$\,0.31 & 97.76 & 0.108$_{-0.006}^{+0.012}$ & 0.44\,$\pm$\,0.04 & 0.96\,$\pm$\,0.10 & 3349\,$\pm$\,142 & 0 (adopted) & (17) \\ 
TOI-811b & 59.9$_{-8.6}^{+13.0}$ & 1.26\,$\pm$\,0.06 & 25.17 & 0.509\,$\pm$\,0.075 & 1.32$_{-0.07}^{+0.05}$ & 1.27$_{-0.09}^{+0.06}$ & 6107\,$\pm$\,77 & 0.40$_{-0.09}^{+0.07}$ & (14) \\ 
TOI-263b & 61.6\,$\pm$\,4.0 & 0.91\,$\pm$\,0.07 & 0.56 & 0.017$_{-0.010}^{+0.009}$ & 0.44\,$\pm$\,0.04 & 0.44\,$\pm$\,0.03 & 3471\,$\pm$\,33 & 0.00\,$\pm$\,0.10 & (18) \\ 
KOI-415b & 62.1\,$\pm$\,2.7 & 0.79$_{-0.07}^{+0.12}$ & 166.79 & 0.689\,$\pm$\,0.000 & 0.94\,$\pm$\,0.06 & 1.25$_{-0.10}^{+0.15}$ & 5810\,$\pm$\,80 & -0.24\,$\pm$\,0.11 & (19) \\ 
WASP-30b & 62.5\,$\pm$\,1.2 & 0.95$_{-0.02}^{+0.03}$ & 4.16 & 0 (fixed) & 1.25$_{-0.04}^{+0.03}$ & 1.39\,$\pm$\,0.03 & 6202$_{-51}^{+42}$ & 0.08$_{-0.05}^{+0.07}$ & (20) \\ 
LHS 6343c & 62.7\,$\pm$\,2.4 & 0.83\,$\pm$\,0.02 & 12.71 & 0.056\,$\pm$\,0.032 & 0.37\,$\pm$\,0.01 & 0.38\,$\pm$\,0.01 & 3130\,$\pm$\,20 & 0.04\,$\pm$\,0.08 & (21) \\ 
CoRoT-15b & 63.3\,$\pm$\,4.1 & 1.12$_{-0.15}^{+0.30}$ & 3.06 & 0 (fixed) & 1.32\,$\pm$\,0.12 & 1.46$_{-0.14}^{+0.31}$ & 6350\,$\pm$\,200 & 0.10\,$\pm$\,0.20 & (22) \\ 
TOI-569b & 64.1$_{-1.4}^{+1.9}$ & 0.75\,$\pm$\,0.02 & 6.56 & 0.002$_{-0.001}^{+0.002}$ & 1.21\,$\pm$\,0.05 & 1.48\,$\pm$\,0.03 & 5768$_{-92}^{+110}$ & 0.29$_{-0.08}^{+0.09}$ & (11) \\ 
EPIC 201702477b & 66.9\,$\pm$\,1.7 & 0.76\,$\pm$\,0.07 & 40.74 & 0.228\,$\pm$\,0.003 & 0.87\,$\pm$\,0.03 & 0.90\,$\pm$\,0.06 & 5517\,$\pm$\,70 & -0.16\,$\pm$\,0.05 & (23) \\ 
LP261-75b & 68.1\,$\pm$\,2.1 & 0.90\,$\pm$\,0.01 & 1.88 & <0.007 & 0.30\,$\pm$\,0.01 & 0.31\,$\pm$\,0.00 & 3100\,$\pm$\,50 & ... & (24) \\ 
NGTS-7Ab & 75.5$_{-13.7}^{+3.0}$ & 1.38$_{-0.14}^{+0.13}$ & 0.68 & 0 (fixed) & 0.24\,$\pm$\,0.03 & 0.61\,$\pm$\,0.06 & 3359$_{-89}^{+106}$ & 0.00\,$\pm$\,0.10 & (25) \\ 
KOI-189b & 78.6\,$\pm$\,3.5 & 1.00\,$\pm$\,0.02 & 30.36 & 0.275\,$\pm$\,0.004 & 0.76\,$\pm$\,0.05 & 0.73\,$\pm$\,0.02 & 4952\,$\pm$\,40 & -0.12\,$\pm$\,0.10 & (26) \\ 
TOI-148b & 77.1$_{-4.6}^{+5.8}$ & 0.81$_{-0.06}^{+0.05}$ & 4.87 & 0.005$_{-0.004}^{+0.006}$ & 0.97$_{-0.09}^{+0.12}$ & 1.20\,$\pm$\,0.07 & 5990\,$\pm$\,140 & -0.24\,$\pm$\,0.25 & this work \\ 
TOI-587b & 81.1$_{-7.0}^{+7.1}$ & 1.32$_{-0.06}^{+0.07}$ & 8.04 & 0.051$_{-0.036}^{+0.049}$ & 2.33\,$\pm$\,0.12 & 2.01\,$\pm$\,0.09 & 9800\,$\pm$\,200 & 0.08$_{-0.12}^{+0.11}$ & this work \\ 
TOI-746b & 82.2$_{-4.4}^{+4.9}$ & 0.95$_{-0.06}^{+0.09}$ & 10.98 & 0.199\,$\pm$\,0.003 & 0.94$_{-0.08}^{+0.09}$ & 0.97$_{-0.03}^{+0.04}$ & 5690\,$\pm$\,140 & -0.02\,$\pm$\,0.23 & this work \\ 
EBLM J0555-57Ab & 87.9\,$\pm$\,4.0 & 0.82$_{-0.06}^{+0.13}$ & 7.76 & 0.089\,$\pm$\,0.004 & 1.18\,$\pm$\,0.08 & 1.00$_{-0.07}^{+0.14}$ & 6386\,$\pm$\,124 & -0.04\,$\pm$\,0.14 & (27) \\ 
TOI-681b & 88.7$_{-2.3}^{+2.5}$ & 1.52$_{-0.15}^{+0.25}$ & 15.78 & 0.093$_{-0.019}^{+0.022}$ & 1.54$_{-0.05}^{+0.06}$ & 1.47\,$\pm$\,0.04 & 7440$_{-140}^{+150}$ & -0.08\,$\pm$\,0.05 & this work \\ 
OGLE-TR-123b & 89.0\,$\pm$\,11.5 & 1.29\,$\pm$\,0.09 & 1.80 & 0 (fixed) & 1.29\,$\pm$\,0.26 & 1.55\,$\pm$\,0.10 & 6700\,$\pm$\,300 & ... & (28) \\ 
TOI-694b & 89.0\,$\pm$\,5.3 & 1.11\,$\pm$\,0.02 & 48.05 & 0.521\,$\pm$\,0.002 & 0.97$_{-0.04}^{+0.05}$ & 1.00\,$\pm$\,0.01 & 5496$_{-81}^{+87}$ & 0.21\,$\pm$\,0.08 & (29) \\ 
KOI-607b & 95.1$_{-3.4}^{+3.3}$ & 1.09$_{-0.06}^{+0.09}$ & 5.89 & 0.395\,$\pm$\,0.009 & 0.99\,$\pm$\,0.05 & 0.92\,$\pm$\,0.03 & 5418$_{-85}^{+87}$ & 0.38$_{-0.09}^{+0.07}$ & (9) \\ 
J1219-39b & 95.4$_{-2.5}^{+1.9}$ & 1.14$_{-0.05}^{+0.07}$ & 6.76 & 0.055\,$\pm$\,0.000 & 0.83\,$\pm$\,0.03 & 0.81$_{-0.02}^{+0.04}$ & 5412$_{-65}^{+81}$ & -0.21\,$\pm$\,0.07 & (20) \\ 
TOI-1213b & 96.1$_{-3.7}^{+4.6}$ & 1.54$_{-0.59}^{+0.99}$ & 27.21 & 0.499\,$\pm$\,0.003 & 0.97$_{-0.06}^{+0.07}$ & 1.02$_{-0.05}^{+0.04}$ & 5550\,$\pm$\,150 & 0.25$_{-0.15}^{+0.14}$ & this work \\ 
OGLE-TR-122b & 96.3\,$\pm$\,9.4 & 1.17$_{-0.13}^{+0.20}$ & 7.27 & 0.205\,$\pm$\,0.008 & 0.98\,$\pm$\,0.14 & 1.05$_{-0.09}^{+0.20}$ & 5700\,$\pm$\,300 & 0.15\,$\pm$\,0.36 & (30) \\ 
K2-76b & 98.7\,$\pm$\,2.0 & 0.89$_{-0.05}^{+0.03}$ & 11.99 & 0.255$_{-0.006}^{+0.007}$ & 0.96\,$\pm$\,0.03 & 1.17$_{-0.06}^{+0.03}$ & 5747$_{-70}^{+64}$ & 0.01\,$\pm$\,0.04 & (31) \\ 
CoRoT 101186644 & 100.5\,$\pm$\,11.5 & 1.01$_{-0.25}^{+0.06}$ & 20.68 & 0.402\,$\pm$\,0.006 & 1.20\,$\pm$\,0.20 & 1.07\,$\pm$\,0.07 & 6090\,$\pm$\,200 & 0.20\,$\pm$\,0.20 & (32) \\ 
J2343+29Ab & 102.7\,$\pm$\,7.3 & 1.24\,$\pm$\,0.07 & 16.95 & 0.161$_{-0.003}^{+0.002}$ & 0.86\,$\pm$\,0.10 & 0.85$_{-0.06}^{+0.05}$ & 5150$_{-60}^{+90}$ & 0.10\,$\pm$\,0.14 & (33) \\ 
EBLM J0954-23Ab & 102.8$_{-5.9}^{+6.0}$ & 0.98\,$\pm$\,0.17 & 7.58 & 0.042\,$\pm$\,0.001 & 1.17\,$\pm$\,0.08 & 1.23\,$\pm$\,0.17 & 6406\,$\pm$\,124 & -0.01\,$\pm$\,0.14 & (27) \\ 
KOI-686b & 103.4\,$\pm$\,5.1 & 1.22\,$\pm$\,0.04 & 52.51 & 0.556\,$\pm$\,0.004 & 0.98\,$\pm$\,0.07 & 1.04\,$\pm$\,0.03 & 5834\,$\pm$\,100 & -0.06\,$\pm$\,0.13 & (26) \\ 
TIC 220568520b & 107.2\,$\pm$\,5.2 & 1.25\,$\pm$\,0.02 & 18.56 & 0.096\,$\pm$\,0.003 & 1.03\,$\pm$\,0.04 & 1.01\,$\pm$\,0.01 & 5589\,$\pm$\,81 & 0.26\,$\pm$\,0.07 & (29) \\ 
HATS551-016B & 114.7$_{-6.3}^{+5.2}$ & 1.46$_{-0.04}^{+0.03}$ & 2.05 & 0.080\,$\pm$\,0.020 & 0.97$_{-0.06}^{+0.05}$ & 1.22$_{-0.03}^{+0.02}$ & 6420\,$\pm$\,90 & -0.60\,$\pm$\,0.06 & (34) \\ 
OGLE-TR-106b & 121.5\,$\pm$\,22.0 & 1.76\,$\pm$\,0.17 & 2.54 & 0.000\,$\pm$\,0.020 & ... & 1.31\,$\pm$\,0.09 & ... & ... & (35) \\ 
EBLM J1431-11Ab & 126.9$_{-3.9}^{+3.8}$ & 1.45$_{-0.05}^{+0.07}$ & 4.45 & 0 (fixed) & 1.20\,$\pm$\,0.06 & 1.11$_{-0.03}^{+0.04}$ & 6161\,$\pm$\,124 & 0.15\,$\pm$\,0.14 & (27) \\ 
HAT-TR-205-013B & 129.9\,$\pm$\,10.5 & 1.62\,$\pm$\,0.06 & 2.23 & 0.012\,$\pm$\,0.021 & 1.04\,$\pm$\,0.13 & 1.28\,$\pm$\,0.04 & 6295$_{-335}^{+245}$ & ... & (36) \\ 
TIC 231005575b & 134.1\,$\pm$\,3.1 & 1.50\,$\pm$\,0.03 & 61.78 & 0.298$_{-0.001}^{+0.004}$ & 1.04\,$\pm$\,0.04 & 0.99\,$\pm$\,0.05 & 5500\,$\pm$\,85 & -0.44\,$\pm$\,0.06 & (37) \\ 
HATS551-021B & 138.2$_{-5.2}^{+14.7}$ & 1.53$_{-0.08}^{+0.06}$ & 3.64 & 0.060\,$\pm$\,0.020 & 1.10\,$\pm$\,0.10 & 1.20$_{-0.01}^{+0.08}$ & 6670\,$\pm$\,220 & -0.40\,$\pm$\,0.10 & (34) \\ 
EBLM J2017+02Ab & 142.2$_{-6.7}^{+6.6}$ & 1.49$_{-0.10}^{+0.13}$ & 0.82 & 0 (fixed) & 1.10\,$\pm$\,0.07 & 1.20$_{-0.05}^{+0.08}$ & 6161\,$\pm$\,124 & -0.07\,$\pm$\,0.14 & (27) \\ 
KIC 1571511B & 148.1\,$\pm$\,0.5 & 1.74$_{-0.01}^{+0.00}$ & 14.02 & 0.327\,$\pm$\,0.003 & 1.26$_{-0.03}^{+0.04}$ & 1.34\,$\pm$\,0.01 & 6195\,$\pm$\,50 & 0.37\,$\pm$\,0.08 & (38) \\ 
WTS 19g-4-02069B & 149.8\,$\pm$\,6.3 & 1.69\,$\pm$\,0.06 & 2.44 & 0 (fixed) & 0.53\,$\pm$\,0.02 & 0.51\,$\pm$\,0.01 & 3300\,$\pm$\,140 & ... & (39) \\ 
\hline
\end{tabular}
\caption{\textbf{References.}
(1) \citealt{Zhou2019}; 
(2) \citealt{Benni2020}; 
(3) \citealt{Bonomo2015}; 
(4) \citealt{Deleuil2008}; 
(5) \citealt{Siverd2012}; 
(6) \citealt{Irwin2010}; 
(7) \citealt{Hodzic2018}; 
(8) \citealt{Carmichael2019}; 
(9) \citealt{Carmichael2019}; 
(10) \citealt{Diaz2013}; 
(11) \citealt{Carmichael2020}; 
(12) \citealt{Persson2019}; 
(13) \citealt{Subjak2020}; 
(14) \citealt{Carmichael2021}; 
(15) \citealt{Gillen2017}; 
(16) \citealt{Csizmadia2015}; 
(17) \citealt{David2019}; 
(18) \citealt{Palle2021}; 
(19) \citealt{Moutou2013}; 
(20) \citealt{Triaud2013}; 
(21) \citealt{Johnson2011}; 
(22) \citealt{Bouchy2011}; 
(23) \citealt{Bayliss2017}; 
(24) \citealt{Irwin2018}; 
(25) \citealt{Jackman2019}; 
(26) \citealt{Diaz2014}; 
(27) \citealt{vonBoetticher2019}; 
(28) \citealt{Pont2006}; 
(29) \citealt{Mireles2020}; 
(30) \citealt{Pont2005a}; 
(31) \citealt{Shporer2017}; 
(32) \citealt{Tal-Or2013}; 
(33) \citealt{Chaturvedi2016}; 
(34) \citealt{Zhou2014}; 
(35) \citealt{Pont2005b}; 
(36) \citealt{Beatty2007}; 
(37) \citealt{Gill2020};
(38) \citealt{Ofir2012}; 
(39) \citealt{Nefs2013}.
\textbf{Note.} The brown dwarf binary system from \citet{Stassun2006}, triple system from \citet{Triaud2020}, and white dwarf companions are not included.
}
\label{tab:trancomp}
\end{table*}

==> tables/spectra_param_sub2.tex <==
\begin{table*} 
    \centering
    %\hspace*{-1cm}
    \begin{tabular}{cccccc}
        \hline\hline
        Star & $\teff$ & $\feh$ & $\logg$  & $\vsini$ & Source  \\
         &  [K] & dex & [cgs] & [km$^{-1}$] &   \\
        \hline
        TOI-148 & 5836 $\pm$ 286 & -0.28 $\pm$ 0.28 & 4.11 $\pm$ 0.37 & 10.1 $\pm$ 0.8 & CORALIE \\     
        TOI-587 & 10400 $\pm$ 300 & 0.07 $\pm$ 0.12 & 4.20 $\pm$ 0.30 & 34.0 $\pm$ 2.0 & TRES \\
        TOI-681 & 7297 $\pm$ 45 & -0.12 $\pm$ 0.05 & 4.32 $\pm$ 0.14 & 30.8 $\pm$ 0.8 & GALAH DR2 \\
        TOI-746 & 5593 $\pm$ 215 & 0.01 $\pm$ 0.29 &  4.30 $\pm$ 0.29 & 6.1 $\pm$ 1.2 & CORALIE \\ 
        TOI-1213 & 5430 $\pm$ 215 & 0.28 $\pm$ 0.16 & 4.47 $\pm$ 0.26 & 4.0 $\pm$ 1.2 & CORALIE \\ 
        \hline
        
        %Santos CORALIE vsini estimates:
        %TOI-148 & 7.1 $\pm$ 0.8
        %TOI-746 & $<$ 2.5
        %TOI-1213 & $<$ 2.5
    \end{tabular}
    
    \caption{Table of stellar parameters derived from spectra. TOI-148, TOI-746, and TOI-1213 parameters were obtained from CORALIE spectra by combining the analysis results of both SpecMatch-Emp \citep{Yee2017} and with an iSpec \citep{Blanco-Cuaresma2014} analysis. The high temperature of TOI-587 precluded using SpecMatch-Emp and iSpec analysis and we use a separate analysis described in Section \ref{sec:specanal} on the TRES spectra. For TOI-681 we use GALAH DR2 results \citep{Buder2018}. \textbf{We refer the reader to the final adopted parameters for each star presented in tables \ref{tab:TOI-148} - \ref{tab:TOI-1213}}.}

    \label{tab:spectra_param}
\end{table*}

==> tables/transiting_companions_table.tex <==
\begin{table*} 
\centering
List of Published 13-150 \mjup Transiting Companions as of June 2021
\tiny
%\hspace*{-0.25cm}
\begin{tabular}{lccrcccccc}
\hline\hline
Name & M$_{\rm2}$ [\mjup] & R$_{\rm2}$ [\rjup] & $P$ [days] & $ecc$ & M$_{\rm1}$ [\msol] & R$_{\rm1}$ [\rsol] & \teff [K] & \feh & Reference \\

\hline

HATS-70b & 12.9$_{-1.6}^{+1.8}$ & 1.38$_{-0.07}^{+0.08}$ & 1.89 & <0.18 & 1.78\,$\pm$\,0.12 & 1.88$_{-0.07}^{+0.06}$ & 7930$_{-820}^{+630}$ & 0.04$_{-0.11}^{+0.10}$ & (1) \\ 
TOI-1278b & 18.5\,$\pm$\,0.5 & 1.09$_{-0.20}^{+0.24}$ & 14.48 & 0.013\,$\pm$\,0.004 & 0.54\,$\pm$\,0.02 & 0.57\,$\pm$\,0.01 & 3799\,$\pm$\,42 & -0.01\,$\pm$\,0.28 & (2) \\ 
GPX-1b & 19.7\,$\pm$\,1.6 & 1.47\,$\pm$\,0.10 & 1.74 & 0.000\,$\pm$\,0.000 & 1.68\,$\pm$\,0.10 & 1.56\,$\pm$\,0.10 & 7000\,$\pm$\,200 & 0.35\,$\pm$\,0.10 & (3) \\ 
Kepler-39b & 20.1$_{-1.2}^{+1.3}$ & 1.24$_{-0.10}^{+0.09}$ & 21.09 & 0.112\,$\pm$\,0.057 & 1.29$_{-0.07}^{+0.06}$ & 1.40\,$\pm$\,0.10 & 6350\,$\pm$\,100 & 0.10\,$\pm$\,0.14 & (4) \\ 
CoRoT-3b & 21.7\,$\pm$\,1.0 & 1.01\,$\pm$\,0.07 & 4.26 & 0 (fixed) & 1.37\,$\pm$\,0.09 & 1.56\,$\pm$\,0.09 & 6740\,$\pm$\,140 & -0.02\,$\pm$\,0.06 & (5) \\ 
KELT-1b & 27.4\,$\pm$\,0.9 & 1.12$_{-0.03}^{+0.04}$ & 1.22 & 0.010$_{-0.007}^{+0.010}$ & 1.33\,$\pm$\,0.06 & 1.47\,$\pm$\,0.04 & 6516\,$\pm$\,49 & 0.05\,$\pm$\,0.08 & (6) \\ 
NLTT 41135b & 33.7$_{-2.6}^{+2.8}$ & 1.13$_{-0.17}^{+0.27}$ & 2.89 & <0.02 & 0.19$_{-0.02}^{+0.03}$ & 0.21$_{-0.01}^{+0.02}$ & 3230\,$\pm$\,130 & -0.25\,$\pm$\,0.25 & (7) \\ 
WASP-128b & 37.2\,$\pm$\,0.8 & 0.94\,$\pm$\,0.02 & 2.21 & <0.007 & 1.16\,$\pm$\,0.04 & 1.15\,$\pm$\,0.02 & 5950\,$\pm$\,50 & 0.01\,$\pm$\,0.12 & (8) \\ 
CWW 89Ab & 39.2$_{-1.1}^{+0.9}$ & 0.94\,$\pm$\,0.02 & 5.29 & 0.189\,$\pm$\,0.002 & 1.10\,$\pm$\,0.04 & 1.03\,$\pm$\,0.02 & 5755\,$\pm$\,49 & 0.20\,$\pm$\,0.09 & (9) (10) \\ 
KOI-205b & 39.9\,$\pm$\,1.0 & 0.81\,$\pm$\,0.02 & 11.72 & <0.031 & 0.93\,$\pm$\,0.03 & 0.84\,$\pm$\,0.02 & 5237\,$\pm$\,60 & 0.14\,$\pm$\,0.12 & (11) \\ 
TOI-1406b & 46.0$_{-2.7}^{+2.6}$ & 0.86\,$\pm$\,0.03 & 10.57 & 0.026$_{-0.010}^{+0.013}$ & 1.18$_{-0.09}^{+0.08}$ & 1.35\,$\pm$\,0.03 & 6290\,$\pm$\,100 & -0.08\,$\pm$\,0.09 & (12) \\ 
EPIC 212036875b & 52.3\,$\pm$\,1.9 & 0.87\,$\pm$\,0.02 & 5.17 & 0.132\,$\pm$\,0.004 & 1.29$_{-0.06}^{+0.07}$ & 1.50\,$\pm$\,0.03 & 6238$_{-60}^{+59}$ & 0.01\,$\pm$\,0.10 & (10) (13) \\ 
TOI-503b & 53.7\,$\pm$\,1.2 & 1.34$_{-0.15}^{+0.26}$ & 3.68 & 0 (fixed) & 1.80\,$\pm$\,0.06 & 1.70$_{-0.04}^{+0.05}$ & 7650$_{-160}^{+140}$ & 0.30$_{-0.09}^{+0.08}$ & (14) \\ 
TOI-852b & 53.7$_{-1.3}^{+1.4}$ & 0.83\,$\pm$\,0.04 & 4.95 & 0.004$_{-0.003}^{+0.004}$ & 1.32$_{-0.04}^{+0.05}$ & 1.71\,$\pm$\,0.04 & 5768$_{-81}^{+84}$ & 0.33\,$\pm$\,0.09 & (15) \\ 
AD 3116b & 54.2\,$\pm$\,4.3 & 1.02\,$\pm$\,0.28 & 1.98 & 0.146\,$\pm$\,0.024 & 0.28\,$\pm$\,0.02 & 0.29\,$\pm$\,0.08 & 3184\,$\pm$\,29 & 0.16\,$\pm$\,0.10 & (16) \\ 
CoRoT-33b & 59.0$_{-1.7}^{+1.8}$ & 1.10\,$\pm$\,0.53 & 5.82 & 0.070\,$\pm$\,0.002 & 0.86\,$\pm$\,0.04 & 0.94$_{-0.08}^{+0.14}$ & 5225\,$\pm$\,80 & 0.44\,$\pm$\,0.10 & (17) \\ 
RIK 72b & 59.2$_{-6.7}^{+6.8}$ & 3.10\,$\pm$\,0.31 & 97.76 & 0.108$_{-0.006}^{+0.012}$ & 0.44\,$\pm$\,0.04 & 0.96\,$\pm$\,0.10 & 3349\,$\pm$\,142 & 0.00\,$\pm$\,0.10 & (18) \\ 
TOI-811b & 59.9$_{-8.6}^{+13.0}$ & 1.26\,$\pm$\,0.06 & 25.17 & 0.509\,$\pm$\,0.075 & 1.32$_{-0.07}^{+0.05}$ & 1.27$_{-0.09}^{+0.06}$ & 6107\,$\pm$\,77 & 0.40$_{-0.09}^{+0.07}$ & (15) \\ 
TOI-263b & 61.6\,$\pm$\,4.0 & 0.91\,$\pm$\,0.07 & 0.56 & 0.017$_{-0.010}^{+0.009}$ & 0.44\,$\pm$\,0.04 & 0.44\,$\pm$\,0.03 & 3471\,$\pm$\,33 & 0.00\,$\pm$\,0.10 & (19) \\ 
KOI-415b & 62.1\,$\pm$\,2.7 & 0.79$_{-0.07}^{+0.12}$ & 166.79 & 0.689\,$\pm$\,0.000 & 0.94\,$\pm$\,0.06 & 1.25$_{-0.10}^{+0.15}$ & 5810\,$\pm$\,80 & -0.24\,$\pm$\,0.11 & (20) \\ 
WASP-30b & 62.5\,$\pm$\,1.2 & 0.95$_{-0.02}^{+0.03}$ & 4.16 & 0 (fixed) & 1.25$_{-0.04}^{+0.03}$ & 1.39\,$\pm$\,0.03 & 6202$_{-51}^{+42}$ & 0.08$_{-0.05}^{+0.07}$ & (21) \\ 
LHS 6343c & 62.7\,$\pm$\,2.4 & 0.83\,$\pm$\,0.02 & 12.71 & 0.056\,$\pm$\,0.032 & 0.37\,$\pm$\,0.01 & 0.38\,$\pm$\,0.01 & 3130\,$\pm$\,20 & 0.04\,$\pm$\,0.08 & (22) \\ 
CoRoT-15b & 63.3\,$\pm$\,4.1 & 1.12$_{-0.15}^{+0.30}$ & 3.06 & 0 (fixed) & 1.32\,$\pm$\,0.12 & 1.46$_{-0.14}^{+0.31}$ & 6350\,$\pm$\,200 & 0.10\,$\pm$\,0.20 & (23) \\ 
TOI-569b & 64.1$_{-1.4}^{+1.9}$ & 0.75\,$\pm$\,0.02 & 6.56 & 0.002$_{-0.001}^{+0.002}$ & 1.21\,$\pm$\,0.05 & 1.48\,$\pm$\,0.03 & 5768$_{-92}^{+110}$ & 0.29$_{-0.08}^{+0.09}$ & (12) \\ 
EPIC 201702477b & 66.9\,$\pm$\,1.7 & 0.76\,$\pm$\,0.07 & 40.74 & 0.228\,$\pm$\,0.003 & 0.87\,$\pm$\,0.03 & 0.90\,$\pm$\,0.06 & 5517\,$\pm$\,70 & -0.16\,$\pm$\,0.05 & (24) \\ 
LP261-75b & 68.1\,$\pm$\,2.1 & 0.90\,$\pm$\,0.01 & 1.88 & <0.007 & 0.30\,$\pm$\,0.01 & 0.31\,$\pm$\,0.00 & 3100\,$\pm$\,50 & ... & (25) \\ 
NGTS-7Ab & 75.5$_{-13.7}^{+3.0}$ & 1.38$_{-0.14}^{+0.13}$ & 0.68 & 0 (fixed) & 0.24\,$\pm$\,0.03 & 0.61\,$\pm$\,0.06 & 3359$_{-89}^{+106}$ & 0.00\,$\pm$\,0.10 & (26) \\ 
KOI-189b & 78.6\,$\pm$\,3.5 & 1.00\,$\pm$\,0.02 & 30.36 & 0.275\,$\pm$\,0.004 & 0.76\,$\pm$\,0.05 & 0.73\,$\pm$\,0.02 & 4952\,$\pm$\,40 & -0.12\,$\pm$\,0.10 & (27) \\ 
TOI-148b & 77.1$_{-4.6}^{+5.8}$ & 0.81$_{-0.06}^{+0.05}$ & 4.87 & 0.005$_{-0.004}^{+0.006}$ & 0.97$_{-0.09}^{+0.12}$ & 1.20\,$\pm$\,0.07 & 5990\,$\pm$\,140 & -0.24\,$\pm$\,0.25 & this work \\ 
TOI-587b & 81.1$_{-7.0}^{+7.1}$ & 1.32$_{-0.06}^{+0.07}$ & 8.04 & 0.051$_{-0.036}^{+0.049}$ & 2.33\,$\pm$\,0.12 & 2.01\,$\pm$\,0.09 & 9800\,$\pm$\,200 & 0.08$_{-0.12}^{+0.11}$ & this work \\ 
TOI-746b & 82.2$_{-4.4}^{+4.9}$ & 0.95$_{-0.06}^{+0.09}$ & 10.98 & 0.199\,$\pm$\,0.003 & 0.94$_{-0.08}^{+0.09}$ & 0.97$_{-0.03}^{+0.04}$ & 5690\,$\pm$\,140 & -0.02\,$\pm$\,0.23 & this work \\
EBLM J0555-57Ab & 87.9\,$\pm$\,4.0 & 0.82$_{-0.06}^{+0.13}$ & 7.76 & 0.089\,$\pm$\,0.004 & 1.18\,$\pm$\,0.08 & 1.00$_{-0.07}^{+0.14}$ & 6386\,$\pm$\,124 & -0.04\,$\pm$\,0.14 & (28) \\ 
TOI-681b & 88.7$_{-2.3}^{+2.5}$ & 1.52$_{-0.15}^{+0.25}$ & 15.78 & 0.093$_{-0.019}^{+0.022}$ & 1.54$_{-0.05}^{+0.06}$ & 1.47\,$\pm$\,0.04 & 7440$_{-140}^{+150}$ & -0.08\,$\pm$\,0.05 & this work \\ 
OGLE-TR-123b & 89.0\,$\pm$\,11.5 & 1.29\,$\pm$\,0.09 & 1.80 & 0 (fixed) & 1.29\,$\pm$\,0.26 & 1.55\,$\pm$\,0.10 & 6700\,$\pm$\,300 & ... & (29) \\
TOI-694b & 89.0\,$\pm$\,5.3 & 1.11\,$\pm$\,0.02 & 48.05 & 0.521\,$\pm$\,0.002 & 0.97$_{-0.04}^{+0.05}$ & 1.00\,$\pm$\,0.01 & 5496$_{-81}^{+87}$ & 0.21\,$\pm$\,0.08 & (30) \\ 
KOI-607b & 95.1$_{-3.4}^{+3.3}$ & 1.09$_{-0.06}^{+0.09}$ & 5.89 & 0.395\,$\pm$\,0.009 & 0.99\,$\pm$\,0.05 & 0.92\,$\pm$\,0.03 & 5418$_{-85}^{+87}$ & 0.38$_{-0.09}^{+0.07}$ & (10) \\ 
J1219-39b & 95.4$_{-2.5}^{+1.9}$ & 1.14$_{-0.05}^{+0.07}$ & 6.76 & 0.055\,$\pm$\,0.000 & 0.83\,$\pm$\,0.03 & 0.81$_{-0.02}^{+0.04}$ & 5412$_{-65}^{+81}$ & -0.21\,$\pm$\,0.07 & (21) \\ 
OGLE-TR-122b & 96.3\,$\pm$\,9.4 & 1.17$_{-0.13}^{+0.20}$ & 7.27 & 0.205\,$\pm$\,0.008 & 0.98\,$\pm$\,0.14 & 1.05$_{-0.09}^{+0.20}$ & 5700\,$\pm$\,300 & 0.15\,$\pm$\,0.36 & (31) \\ 
TOI-1213b & 97.5$_{-4.2}^{+4.4}$ & 1.66$_{-0.55}^{+0.78}$ & 27.22 & 0.498$_{-0.002}^{+0.003}$ & 0.99$_{-0.06}^{+0.07}$ & 0.99\,$\pm$\,0.04 & 5590\,$\pm$\,150 & 0.25$_{-0.14}^{+0.13}$ & this work \\ 
K2-76b & 98.7\,$\pm$\,2.0 & 0.89$_{-0.05}^{+0.03}$ & 11.99 & 0.255$_{-0.006}^{+0.007}$ & 0.96\,$\pm$\,0.03 & 1.17$_{-0.06}^{+0.03}$ & 5747$_{-70}^{+64}$ & 0.01\,$\pm$\,0.04 & (32) \\ 
CoRoT 101186644 & 100.5\,$\pm$\,11.5 & 1.01$_{-0.25}^{+0.06}$ & 20.68 & 0.402\,$\pm$\,0.006 & 1.20\,$\pm$\,0.20 & 1.07\,$\pm$\,0.07 & 6090\,$\pm$\,200 & 0.20\,$\pm$\,0.20 & (33) \\ 
J2343+29Ab & 102.7\,$\pm$\,7.3 & 1.24\,$\pm$\,0.07 & 16.95 & 0.161$_{-0.003}^{+0.002}$ & 0.86\,$\pm$\,0.10 & 0.85$_{-0.06}^{+0.05}$ & 5150$_{-60}^{+90}$ & 0.10\,$\pm$\,0.14 & (34) \\ 
EBLM J0954-23Ab & 102.8$_{-5.9}^{+6.0}$ & 0.98\,$\pm$\,0.17 & 7.58 & 0.042\,$\pm$\,0.001 & 1.17\,$\pm$\,0.08 & 1.23\,$\pm$\,0.17 & 6406\,$\pm$\,124 & -0.01\,$\pm$\,0.14 & (28) \\ 
KOI-686b & 103.4\,$\pm$\,5.1 & 1.22\,$\pm$\,0.04 & 52.51 & 0.556\,$\pm$\,0.004 & 0.98\,$\pm$\,0.07 & 1.04\,$\pm$\,0.03 & 5834\,$\pm$\,100 & -0.06\,$\pm$\,0.13 & (27) \\ 
TIC 220568520b & 107.2\,$\pm$\,5.2 & 1.25\,$\pm$\,0.02 & 18.56 & 0.096\,$\pm$\,0.003 & 1.03\,$\pm$\,0.04 & 1.01\,$\pm$\,0.01 & 5589\,$\pm$\,81 & 0.26\,$\pm$\,0.07 & (30) \\ 
HATS551-016B & 114.7$_{-6.3}^{+5.2}$ & 1.46$_{-0.04}^{+0.03}$ & 2.05 & 0.080\,$\pm$\,0.020 & 0.97$_{-0.06}^{+0.05}$ & 1.22$_{-0.03}^{+0.02}$ & 6420\,$\pm$\,90 & -0.60\,$\pm$\,0.06 & (35) \\ 
OGLE-TR-106b & 121.5\,$\pm$\,22.0 & 1.76\,$\pm$\,0.17 & 2.54 & 0.000\,$\pm$\,0.020 & ... & 1.31\,$\pm$\,0.09 & ... & ... & (36) \\ 
EBLM J1431-11Ab & 126.9$_{-3.9}^{+3.8}$ & 1.45$_{-0.05}^{+0.07}$ & 4.45 & 0 (fixed) & 1.20\,$\pm$\,0.06 & 1.11$_{-0.03}^{+0.04}$ & 6161\,$\pm$\,124 & 0.15\,$\pm$\,0.14 & (28) \\ 
HAT-TR-205-013B & 129.9\,$\pm$\,10.5 & 1.62\,$\pm$\,0.06 & 2.23 & 0.012\,$\pm$\,0.021 & 1.04\,$\pm$\,0.13 & 1.28\,$\pm$\,0.04 & 6295$_{-335}^{+245}$ & ... & (37) \\ 
TIC 231005575b & 134.1\,$\pm$\,3.1 & 1.50\,$\pm$\,0.03 & 61.78 & 0.298$_{-0.001}^{+0.004}$ & 1.04\,$\pm$\,0.04 & 0.99\,$\pm$\,0.05 & 5500\,$\pm$\,85 & -0.44\,$\pm$\,0.06 & (38) \\ 
HATS551-021B & 138.2$_{-5.2}^{+14.7}$ & 1.53$_{-0.08}^{+0.06}$ & 3.64 & 0.060\,$\pm$\,0.020 & 1.10\,$\pm$\,0.10 & 1.20$_{-0.01}^{+0.08}$ & 6670\,$\pm$\,220 & -0.40\,$\pm$\,0.10 & (35) \\ 
EBLM J2017+02Ab & 142.2$_{-6.7}^{+6.6}$ & 1.49$_{-0.10}^{+0.13}$ & 0.82 & 0 (fixed) & 1.10\,$\pm$\,0.07 & 1.20$_{-0.05}^{+0.08}$ & 6161\,$\pm$\,124 & -0.07\,$\pm$\,0.14 & (28) \\ 
KIC 1571511B & 148.1\,$\pm$\,0.5 & 1.74$_{-0.01}^{+0.00}$ & 14.02 & 0.327\,$\pm$\,0.003 & 1.26$_{-0.03}^{+0.04}$ & 1.34\,$\pm$\,0.01 & 6195\,$\pm$\,50 & 0.37\,$\pm$\,0.08 & (39) \\ 
WTS 19g-4-02069B & 149.8\,$\pm$\,6.3 & 1.69\,$\pm$\,0.06 & 2.44 & 0 (fixed) & 0.53\,$\pm$\,0.02 & 0.51\,$\pm$\,0.01 & 3300\,$\pm$\,140 & ... & (40) \\ 
\hline
\end{tabular}
\begin{tablenotes}
\item \textbf{References. }
\tiny
(1) \citealt{Zhou2019};
(2) \citealt{Artigau2021}; 
(3) \citealt{Benni2020}; 
(4) \citealt{Bonomo2015}; 
(5) \citealt{Deleuil2008}; 
(6) \citealt{Siverd2012}; 
(7) \citealt{Irwin2010}; 
(8) \citealt{Hodzic2018}; 
(9) \citealt{Nowak2017}; 
(10) \citealt{Carmichael2019}; 
(11) \citealt{Diaz2013}; 
(12) \citealt{Carmichael2020}; 
(13) \citealt{Persson2019}; 
(14) \citealt{Subjak2020}; 
(15) \citealt{Carmichael2021}; 
(16) \citealt{Gillen2017}; 
(17) \citealt{Csizmadia2015}; 
(18) \citealt{David2019}; 
(19) \citealt{Palle2021}; 
(20) \citealt{Moutou2013}; 
(21) \citealt{Triaud2013}; 
(22) \citealt{Johnson2011}; 
(23) \citealt{Bouchy2011}; 
(24) \citealt{Bayliss2017}; 
(25) \citealt{Irwin2018}; 
(26) \citealt{Jackman2019}; 
(27) \citealt{Diaz2014}; 
(28) \citealt{vonBoetticher2019}; 
(29) \citealt{Pont2006}; 
(30) \citealt{Mireles2020}; 
(31) \citealt{Pont2005a}; 
(32) \citealt{Shporer2017}; 
(33) \citealt{Tal-Or2013}; 
(34) \citealt{Chaturvedi2016}; 
(35) \citealt{Zhou2014}; 
(36) \citealt{Pont2005b}; 
(37) \citealt{Beatty2007}; 
(38) \citealt{Gill2020};
(39) \citealt{Ofir2012}; 
(40) \citealt{Nefs2013}.
\textbf{Note.} The brown dwarf binary system from \citet{Stassun2006}, triple system from \citet{Triaud2020}, and white dwarf companions are not included.
\end{tablenotes}

\caption{\tiny List of Published 13-150 \mjup Transiting Companions as of June 2021}
\label{tab:trancomp}
\end{table*}
